Parameter Hub: a Rack-Scale Parameter Server for Distributed Deep Neural Network Training

Distributed deep neural network (DDNN) training constitutes an increasingly important workload that frequently runs in the cloud. Larger DNN models and faster compute engines are shifting DDNN training bottlenecks from computation to communication. This paper characterizes DDNN training to precisely pinpoint these bottlenecks. We found that timely training requires high performance parameter servers (PSs) with optimized network stacks and gradient processing pipelines, as well as server and network hardware with balanced computation and communication resources. We therefore propose PHub, a high performance multi-tenant, rack-scale PS design. PHub co-designs the PS software and hardware to accelerate rack-level and hierarchical cross-rack parameter exchange, with an API compatible with many DDNN training frameworks. PHub provides a performance improvement of up to 2.7x compared to state-of-the-art distributed training techniques for cloud-based ImageNet workloads, with 25% better throughput per dollar.

==> DesignExploration.tex <==


%% \subsection{Other points in the design space}


%% \subsubsection{Centralized versus Sharded}

%% It is common supports running its parameter server in either a a centralized way or 
%% and PSLite support running th
%% The PHub 
%% We described the PHub as a centralized design, running on a dedicated machine. Many other parameter exchange mechanisms use a sharded approach, with multiple paramater server machines each holding a shard of the model; the PHub can be used in this way as well.

%% It is common to colocate the shards on the workers, under the assumption that .

%% \subsection{Central PS versus Sharded PS}
%% The following analysis assumes there are N workers participating distributed training, and each of them produces gradient of size W in each batch, and we ignore colocation effects. We assume it takes T unit of time to transfer W from worker (worker bandwidth is thus $\frac{W}{T}$). We focus on three metrics regarding communication overhead: the total number of messages sent per batch, communication latency for each batch, and total data movement. We define total data movement as the sum of bytes moved along each segment of physical wires, and if the same piece of data travels along multiple segments of wires (like through a switch), it is counted only once.

%% During parameter synchronization, central parameter servers minimizes the number of messages sent to $2N$ per key per batch (N push messages and N response messages) and has a total data movement of $2NW$. If enough bandwidth is available on the parameter server, the communication latency would be $2T$ per key per batch. Central parameter achieves optimality in all three considered metrics. But as previous works pointed out, it can suffer from incast congestions as the load of work (communication and computation) increases linearly with the number of workers. Thus central parameter server does not often scale well with number with worker nor with depth of neural networks without proper balanced design.

%% One alleviation to the scaling problem in central parameter servers is to shard it. While there can be many physical sharding strategies, we focus our discussion to naive, ring and tree sharding. 

%% In naive sharing, a central parameter server is partitioned into physically disjoint parts, each serving a subset of keys in the parameter space independently. This is logically equivalent to a more powerful central parameter server with multiple interfaces and achieves the same optimality in terms of messages sent, communication latency and data movement per batch. Naive sharing however requires additional hardware resources and is more subject to delays in the network and stragglers in the parameter server shards. Similar to central parameter server, naive sharding requires linearly more hardware resources to scale system throughput with the number of workers.


%% A sharded parameter server can be logically organized as a ring, where each shard usually colocates with a worker. Gradients of each key are passed along the ring, performing aggregation with the gradient of the key on the current hop of the ring, and passing the aggregated buffer down the ring. A ring sharded parameter server trades communication latency for computation and smaller bandwidth requirement, because aggregation is distributed at each hop and only the aggregated buffer is sent out. Ring parameter servers cost $2N$ messages per key per batch, and a total data movement of $2NW$, but has latency of $2NT$. Ring parameter server removes the need for dedicated server hardware, but its latency (O($N$))scales linearly with the number of workers, which can be very harmful to the system throughput, especially for smaller neural networks. Ring parameter servers are generally not used in practice.

%% Another option is a reduction tree of parameter server shards. In this setup, a parameter server shard (which is a tree node) aggregates the gradients from all its children, and passes the aggregated buffer up the tree. The root then contains the final result. A reduction tree has the same merit of reduced bandwidth usage but significant reduced latency of $O(logN)$ at the cost of additional messages and more total data movement: In the special case of fan out 2, each key requires $4N$ messages per batch, with a latency of $2logNT$ and the total data movement is $4NW$. However, a reduction tree requires a special physical network layout to be implemented efficiently.



%% \subsection{Sharding and Colocation}
%% We have described the PHub as a centralized parameter server running on dedicated hardware. If a single PHub does not provide enough throughput, it may be scaled by sharding the model amongst multiple PHubs, still running on dedicated hardware.

%% Another common point in the design space is to colocate parameter server shards with workers. This increases the per-machine bandwidth requirement:
%% A sharded, non-colocated design with $N$ workers and a model size of $W$ requires each worker process to send $NW$ bytes, and each shard

%%  to send messages sent to $2N$ per key per batch (N push messages and N response messages) and has a total data movement of $2NW$. If enough bandwidth is 
%% One commonly-used trick to reduce total data movement in sharded parameter servers is to colocate servers and workers. For example, in naive sharding with colocation, a worker does not need to send keys processed by the local server shard through the network, saving a total of $1/N$ amount of data movement if each server is sharded with a worker.

%% However, modern training frameworks overlap computation of backward pass with synchronization, and this means that the parameter server process and the worker training process will contend for computation as well as communication resources, thus if caution is not taken, the benefit gain from reduced data movement due to colocation will not compensate for the loss of performance due to contention. Consider a shared network interface, with colocation on, the total data transmitted from the single node would be $4W(1-\frac{1}{N})$, versus $2W$ when colocation is off. This near $2x$ data movement for the node is detrimental to training performance.




==> SOCC 18/Abstract.tex <==
\begin{abstract}
% from single-box compute-bound traning  to balancing between compute and communication in distributed training

Distributed deep neural network (DDNN) training constitutes an increasingly important workload that frequently runs in the cloud. Larger DNN models and faster compute engines are shifting DDNN training bottlenecks from computation to communication.
%, stressing the physical network and the parameter server (PS)---a key value store where worker nodes periodically exchange model updates.
% Deep Neural Network training with stochastic gradient descent is often seen as a compute-bound problem, best done in a single large compute node with many GPUs. However, as DNNs get bigger, timely training requires exploiting parallelism with a distributed training system. This is typically done using parameter servers---key-value stores that hold the central model---and worker nodes that send parameter updates to the servers after processing input training data.  This system organization lends itself to a rich design space of where to map computation, how to distribute model data, and how to balance compute, communication and memory resource usage. 
This paper characterizes DDNN training to precisely pinpoint these bottlenecks. We found that timely training requires high performance parameter servers (PSs) with optimized network stacks and gradient processing pipelines, as well as server and network hardware with balanced computation and communication resources. We therefore propose \phub, a high performance multi-tenant, rack-scale PS design. \phub co-designs the PS software and hardware to accelerate rack-level and hierarchical cross-rack parameter exchange, with an API compatible with many DDNN training frameworks. \phub provides a performance improvement of up to 2.7x compared to state-of-the-art distributed training techniques for cloud-based ImageNet workloads, with 25\% better throughput per dollar.

%In this paper we present a comprehensive design space exploration for distributed training. 
%We then propose a new organization and a new entity called the Parameter Hub, which centralizes the model in a single box with balanced bandwidth connections to worker nodes, and performs parameter update aggregation centrally. This significantly reduces network bandwidth needs and enables data locality and synchronization optimizations. We build a prototype of the Parameter Hub system on top of the \mxnet\ training framework and show a performance improvement of up to 3x compared to state-of-the-art distributed training techniques for image classification workloads in cloud environments.

\end{abstract}


==> SOCC 18/Background.tex <==
%\section{Background}
\section{Bottlenecks in Cloud-Based Training}
\label{sec:background}


\begin{figure}
	\includegraphics[width=\linewidth,trim=4 4 4 4,clip]{Figures/DistributedTraining.pdf}
	\caption{A few iterations in distributed training.}
	\label{fig:ddnn}
\end{figure}

% Artificial neural networks offer a biologically-inspired approach to computation. They are programmed to perform a task by learning from a large number of labeled examples in an iterative process called training.

%\subsection{Neural Networks and DDNN Training}

% A neural network consists of a collection of connected layers. Each layer performs some computation; many have state referred to as weights or parameters. The weights for a layer
% can range from a few bytes to tens of megabytes. The combination of all layers' weights comprises the model.

Modern neural networks can have hundreds of \textit{layers} making up multi-megabyte-size \textit{models}.% (or sets of weights or parameters).
The training process has three phases. In the \textit{forward pass}, a prediction is generated for an input. In the \textit{backward pass}, the prediction is compared with a label to calculate prediction error; then, through \textit{backpropagation}~\cite{backprop}, the gradient for each parameter %of each layer 
is calculated with respect to this error. The model is then \textit{updated} using these gradients, often using a variant of the gradient descent optimization algorithm. Computation is often done on GPUs or other accelerators suited to regular data-parallel operations, processing tens to hundreds of samples at once (\emph{minibatching}).
%Multiple examples are processed in each GPU simultaneously in a single \emph{minibatch} which typically contains tens to hundreds of samples. 
%Each GPU processes multiple examples simultaneously in a \emph{minibatch} which typically contains tens to hundreds of samples. 

The distributed training process (Figure~\ref
{fig:ddnn}) % differs from the non-distributed one in a few key ways. 
is different in a few ways.
%First, a mean gradient is calculated for each minibatch in each GPU. %
First, a mean gradient is calculated across all minibatches in all the GPUs in each machine. Then, the mean of the gradients from each machine is calculated. Finally, the model is updated based on that mean, new parameters are broadcast to each machine and GPU, and the next batch is trained. This paper focuses on optimizing calculation for both the mean gradient across machines and subsequent model updates (or \textit{parameter exchange}).

%Two techniques are commonly used to do parameter exchange. In the first, 
In a typical DDNN training setup, machines can take the role of a worker and/or a parameter server (PS). PSs are specialized key-values stores that collect the gradients and update the model~\cite{ps0,ps1,ps2,ps3}. In this paper, we use ``key'' to refer to a layer, and ``value'' to refer to the set of parameters for that layer. 

%n the second, each worker also stores a shard or replica of the global model; model updates are done through collective communication operations involving all machines.

The process described here is \emph{synchronous training}, where all machines and GPUs execute a new minibatch simultaneously and update the model based on the gradients in the current iteration. It is also possible to train asynchronously~\cite{tensorflow,revisitSGD,GeePS,recht2011hogwild,projectAdam,googleDNN} or with relaxed consistency~\cite{DBLP:journals/corr/DaiKWHGX14,SSP,BSP,184014,Wei:2015:MCC:2806777.2806778}, sacrificing reproducibility for potential throughput increase. %updating the model with the gradient from each GPU's minibatch with little or no synchronization among machines; this can improve throughput in some situations but may limit repeatability and debuggability. 
We focus on synchronous training due to its simplicity and commonality in industry, but our techniques can also benefit asynchronous training.


\begin{figure}[tb!]
	\includegraphics[width=\linewidth,trim=1 5 1 0,clip]{Figures/PSSetups.pdf}
	\caption{PS configurations in a DDNN training system, and minimum network bandwidth to fully hide communication overhead.}
	\label{fig:pssetups}
\end{figure}



\subsection{Common PS Configurations}
PS configurations primarily differ along two axes: colocated (C) versus non-colocated (NC), and centralized (C) versus sharded (S). %In a colocated setting, a PS process can run with worker processes in the same machine. In a non-colocated setting, a machine is dedicated to a worker or a PS process.  
A PS setup is colocated if a worker and a server process share the same physical machine. A PS setup is centralized if a single PS process handles all keys; and a sharded setup load-balances keys across multiple PS processes.
%A centralized PS stores the entire model, whereas each sharded PS stores only a partition of the keys in the entire key space. The size of each partition is usually balanced by the available hardware resources. 
During synchronization, each worker sends and receives model updates from each PS process. Figure \ref{fig:pssetups} illustrates the four combinations of choices from these two axes: Colocated Centralized (CC), Colocated Sharded (CS), Non-colocated Centralized (NC) and Non-colocated Sharded (NCS).

In general, sharded PSs scale better at higher hardware costs. Colocated PSs reduce total data movement on the network by $\frac{1}{N}$ with $N$ workers participating: the update for the partition of the model assigned to a colocated PS need not go through the network. While many frameworks default to CS configurations~\cite{MXNetont0:online, Distribu25:online}, in a colocated setup the PS process interferes with the training process, because both are contending for network and processing resources. Specifically, compared to NC PSs, \textit{each network interface must process roughly 2x the network traffic, because both the colocated worker and PS processes must send and receive model updates from remote hosts}, creating a major bottleneck in network-bound DDNN training. 

\subsection{The \mxnet Framework}

\mxnet\cite{chen2015mxnet} is a widely used, state-of-the-art DDNN training framework that supports many new optimizations in the literature~\cite{poseidon,chen2016training,GeePS}. It is widely used on AWS~\cite{ApacheMX19:online}, and natively supports distributed training: its PS implementation relies on TCP, built on top of the ZMQ~\cite{zmq} distributed messaging library.

All modern DNN training frameworks can fully utilize GPU resources by taking advantage of primitives, such as CuDNN. These frameworks offer comparable throughput when training DNNs. For distributed training, many frameworks such as \mxnet provide eager scheduling of parameter exchanges, overlapping backward computation with parameter synchronization, hiding communication latency. We measured distributed training performance and scalability for Caffe2, TensorFlow, and \mxnet{}\footnote{Caffe2: Halving and doubling. TensorFlow and \mxnet: CS PSs with a 1:1 worker-to-PS ratio. Network: 56 Gbps IPoIB. GPU: GTX 1080 Ti. Neural Network: ResNet 50 with batch size of 32. Poseidon hangs when more than 5 workers training this network in our cluster. 8-worker throughput is overestimated as per worker throughput (at 5 workers) * 8.} 
with up to 8 worker nodes. We found comparable throughput when training ResNet 50 on a 56 Gbps network using SGD, with \mxnet slightly leading the pack (Table \ref{table:frameworkPerf}). These results align well with other observations \cite{Chainer,1608.07249,zhudnn}. Therefore, we use \mxnet as the basis for our implementations and optimizations, but the techniques are generalizable.


\begin{table}[tb!]
        \centering
        \footnotesize
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		   & Local & 2 nodes & 4 nodes & 8 nodes\\
		\hline 
		TensorFlow   & 152  &  213  & 410    &  634 \\
		\hline
		Caffe2 & 195   &  266  &  343   &   513  \\
		\hline
		TF+Poseidon\cite{poseidon} & 209 & 229  & 364 & $<$648 \\
		\hline
		\mxnet & 190  &  187  &  375   &  \textbf{688}  \\
		\hline
	\end{tabular}
	\caption{Throughput (samples/s) of major DNN training frameworks with a 56 Gbps network.}
	\label{table:frameworkPerf}
\end{table}





%\begin{table}[ht!]
%	\centering
%	\begin{tabular}{|c|c|}
%		\hline
%		Setup   & Bandwidth Requirement\\
%		\hline 
%		CC     &  $2M(N-1)/t$\\
%		\hline
%		CS & $4M(N-1)/Nt$ \\
%		\hline
%		NCC &  $2MN/t$ \\
%		\hline
%		NCS & $2M/t$ \\
%		\hline
%	\end{tabular}
%	\caption{Analytical per machine lower bound estimates of network bandwidth to fully hide communication latency.}
%	\label{table:bwReqAnalytical}
%\end{table}





==> SOCC 18/Characterization.tex <==
%\section{Bottlenecks in Cloud-Based Training}
\subsection{Bottleneck Findings}
\label{sec:cloudTraining}
Ideally, communication latency is fully hidden by computation, i.e., compute engines never wait for data. In reality, since computation speed exceeds communication speed in cloud-based DDNN training, time is wasted waiting for model updates (Figure \ref{fig:IncreasingCommToCompRatio}). Workers run much faster locally~(Table \ref{table:frameworkPerf}), so the bottlenecks must lie in the PS, the network stack, and/or the physical network itself. Our study finds three major bottlenecks in cloud-based DDNN training: insufficient network bandwidth, framework inefficiencies, and suboptimal deployment in the cluster. We elaborate on each below. 

\subsubsection{Insufficient Bandwidth}
%We profiled with \mxnet multiple DNNs of different model sizes and computation-to-communication ratios in a varying bandwidth environment.
%Using \mxnet, 
We profiled the training of multiple DNNs of different model sizes and computation-to-communication ratios. %, while varying network bandwidth.
Our setup used 8 workers and 8 CS PSs.
%First, the available machine instances on the cloud lacked sufficient bandwidth.
We observed \textit{it was nearly impossible to eliminate communication latency in cloud-based training due to limited network bandwidth.}
We estimated the minimum bandwidth requirement to fully hide communication latency in the network as follows: given a model size of $M$, and $T$ time for each iteration, with $N$ workers participating, the network should at least be able to send and receive model updates within the computation time (assuming infinitely fast PSs and that sending/receiving could fully overlap). Figure \ref{fig:pssetups} gives an analytical lower bound of \textit{per host bandwidth}, and Table \ref{table:bwReqDC} shows the required bandwidth for various DNNs: DNNs demand more bandwidth than mainstream cloud providers offer (typically 10-25 Gbps) in the VMs. %\TODO{Fig 4 shows an expression, the table shows an actual number, make it clear the table what the BW requirement is and what the measured BW was.} %It is worth noting that CS PSs have indeed 2x bandwidth demand than their NCS counterpart.
A similar observation was made in prior work~\cite{alannetwork, zhudnn}. Furthermore, bandwidth requirement increases with worker count.

\subsubsection{Framework Bottlenecks}
However, even with ample communication resources, existing PSs failed to hide communication latency and struggled to scale. Table \ref{table:frameworkPerf} shows that all major DNN training frameworks %failed to achieve 50\% scaling on a 56Gbps IPoIB network (112Gbps bidirectional) in our cluster with 8 workers and PSs. 
do not scale well with a 56 Gbps IPoIB network.
We investigated the cause for \mxnet by breaking down the overhead for each major component of a training iteration (legends of Figure \ref{fig:overheadBreakdown}). Since all stages overlap one another, and since ideally we would like early stages to fully hide the latency of later stages, we show \textit{progressive overhead} in Figure \ref{fig:overheadBreakdown}: we gradually turned on different components in the \mxnet DDNN training pipeline, and each segment shows the \textit{additional overhead that previous stages could not hide}. Specifically, the compute segment shows how long the GPU is active; the data copy segment shows the additional overhead of turning on distributed training without aggregation and optimization; the aggregation and optimization segments show additional overheads of enabling them in that order; and the ``other'' overheads segment includes synchronization and overheads that are not specific to a single component. We explain the high overhead for some components:

\begin{table}
        \centering
        \footnotesize
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Network   & CC & CS & NCC & NCS\\
		\hline
		ResNet 269    & 122   & 31   & 140    &  17   \\
		\hline
		Inception & 44   &  11  &  50   &  6  \\
		\hline
		GoogleNet & 40   &  10  &  46   &  6  \\
	
		\hline 
		AlexNet   & 1232  &  308  & 1408    &  176  \\
		\hline
	\end{tabular}
	\caption{Estimated bisection bandwidth (Gbps) lower bound on the PS side for hiding communication latency. Same setup as Table \ref{table:frameworkPerf}.}
	\label{table:bwReqDC}
\end{table}


%\begin{CompactItemize}
	\noindent\textbf{Data copy:} each layer's parameters were copied to and from OS buffers 4 times during parameter exchange.
\vspace{-0.1ex}	

	\noindent \textbf{Aggregation and optimization:} \mxnet's ``wide'' approach to achieving parallelism did not achieve high throughput in our measurements (see \mysection\ref{sec:tallvswide}). 
\vspace{-0.1ex}	
	
	\noindent \textbf{Synchronization:} \mxnet's dispatcher thread needs to synchronize access with ZMQ threads, aggregation threads and a optimization thread via shared queues, leading to bad locality and increased synchronization overhead. 
	%to a shared queue; that dispatcher thread then performs aggregation and sends the data to another group of OpenMP threads for optimization. Inter-thread interactions and shared structure accesses increase overhead.
%\end{CompactItemize}
%% We now explain the high overhead of some components.

%% \vspace{0.05in}
%% \noindent \textbf{Data copy:} each layer's parameters were copied to and from OS buffers 4 times during parameter exchange, leading to inefficiencies.

%% \vspace{0.05in}
%% \noindent \textbf{Aggregation and Optimization:} \mxnet's ``wide'' approach to achieving parallelism did not achieve high throughput in our measurement (see \mysection\ref{sec:tallvswide}). 

%% \vspace{0.05in}
%% \noindent \textbf{Synchronization:} \mxnet's dispatcher thread needs to synchronize access with ZMQ threads to a shared queue; that dispatcher thread then performs aggregation, and sends the data to another group of OpenMP threads for optimization. Inter-thread interactions and shared structure accesses cause high overhead.
\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=3 2 2 4,clip]{Figures/OverheadBreakdown.pdf}
	\caption{Progressive overhead breakdown of different stages during the distributed training pipeline for \mxnet DDNN training on a 56Gbps network. Link capacity accounts for a small fraction of the copy and communication overhead in this setting.}
	\label{fig:overheadBreakdown}
\end{figure}

\begin{figure}[t!]
	\centering
	\includegraphics[width=.7\linewidth,trim=2 1 1 2,clip]{Figures/ShardDeployment.pdf}
	\caption{When workers/servers span multiple racks in cloud-based training, large delay occurs due to gradient update traffic going through an oversubscribed network core.}
	\label{fig:deploymentOverhead}
\end{figure}

%% \begin{figure}[t!]
%% 	\centering
%% 	\includegraphics[width=.7\linewidth,trim=2 1 1 2,clip]{Figures/BWHeatmap.pdf}
%% 	\caption{Pairwise bandwidth of P2.8xLarge instances. 8 Machines seem to form two clusters.}
%% 	\label{fig:bWHeatmap}
%% \end{figure}

\subsubsection{Deployment-related Overhead}
VMs associated with a training job can be far away from each other when launched in the cloud. Existing frameworks assume homogeneous inter-VM bandwidths, which results in excessive communications between distant VMs, in turn leading to bottlenecks.
We conducted an experiment to probe pair-wise bandwidth of 8 P2.8xLarge 10 Gbps instances on EC2 and found that bandwidths can vary by a factor of 2---even between send and receive streams of the same instance pair.
Some cloud environments support co-scheduling constraints (e.g., EC2 placement groups), but for large jobs on busy clusters it may take a long time to satisfy these constraints.


%Figure \ref{fig:deploymentOverhead} illustrates such an example where half of the gradient update is cross-rack traffic in a CS setting.


One possible reason is the oversubscribed network topology in the data center~\cite{Mysore2009PortLandAS,Roy2015InsideTS, incbricks}, providing full bisection bandwidth within each rack but not across racks when the core is busy. Thus, gradient update streams that go through a potentially oversubscribed network core~\cite{vl2-a-scalable-and-flexible-data-center-network,43837} can be delayed. Network topology awareness is crucial for DDNN workloads~\cite{DBLP:journals/corr/abs-1712-03890, wang2018optimal}.
%All PS setups suffer from this problem in the cloud, as there is little or no control\footnote{Mechanism such as placement group~\cite{Placemen61:online} exists, but fitting all machines in one placement group creates scheduling problems.} on where VMs are physically located.
In our work, we pursue a rack-scale PS that takes advantage of intra-rack full bisection bandwidth and minimizes inter-rack traffic via \textit{hierarchical reduction algorithms} (see Section \ref{sec:hierarchicalReduction}). 



==> SOCC 18/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We found that inefficient PS software architecture and network environment-induced overhead were the major bottlenecks of distributed training with modern GPUs in the cloud, making DDNN training a communication-bound workload. To eliminate these bottlenecks, we proposed \phub, a high performance multi-tenant, rack-scale PS design, with co-designed software and hardware to accelerate rack-level and hierarchical cross-rack parameter exchange. Our evaluation showed that \phub provides up to 2.7x higher throughput, with 25\% better throughput per dollar.


%% To eliminate these bottlenecks, we proposed the \phub software, which uses an optimized network stack and a streamlined gradient processing pipeline. We also prototyped \phubbox, a balanced hardware design for a rack-scale, centralized parameter servers that fully utilizes \phub. We showed that our system can provide a throughput benefit of over 3x when compared to the state-of-the-art in DDNN training.





%We provide a comprehensive design exploration of distributed deep neural network training systems. 
%We observe that current trends in deep learning model size and training computational cost contrasted with projections in computing performance, memory bandwidth and network bandwidth point to the need of balancing computation and communication for efficient training. Based on those observations and the design exploration, we proposed \phub, a new system architecture that physically centralizes parameters to enable more efficient communication, locality and synchronization optimization in a scalable fashion. We found a single \phub is capable of supporting an entire cluster of workers. Our \phub prototype is effective in accelerating deep neural network training in all physical network conditions, and can provide 3x faster training throughput compared to the state-of-the-art. 

%These results suggest that being able to move application-level computation and storage to  the network infrastructure can enable fundamentally more efficient system designs. Future programmable switch architectures can enable that vision. 


==> SOCC 18/DesignExploration.tex <==


%% \subsection{Other points in the design space}


%% \subsubsection{Centralized versus Sharded}

%% It is common supports running its parameter server in either a a centralized way or 
%% and PSLite support running th
%% The PHub 
%% We described the PHub as a centralized design, running on a dedicated machine. Many other parameter exchange mechanisms use a sharded approach, with multiple paramater server machines each holding a shard of the model; the PHub can be used in this way as well.

%% It is common to colocate the shards on the workers, under the assumption that .

%% \subsection{Central PS versus Sharded PS}
%% The following analysis assumes there are N workers participating distributed training, and each of them produces gradient of size W in each batch, and we ignore colocation effects. We assume it takes T unit of time to transfer W from worker (worker bandwidth is thus $\frac{W}{T}$). We focus on three metrics regarding communication overhead: the total number of messages sent per batch, communication latency for each batch, and total data movement. We define total data movement as the sum of bytes moved along each segment of physical wires, and if the same piece of data travels along multiple segments of wires (like through a switch), it is counted only once.

%% During parameter synchronization, central parameter servers minimizes the number of messages sent to $2N$ per key per batch (N push messages and N response messages) and has a total data movement of $2NW$. If enough bandwidth is available on the parameter server, the communication latency would be $2T$ per key per batch. Central parameter achieves optimality in all three considered metrics. But as previous works pointed out, it can suffer from incast congestions as the load of work (communication and computation) increases linearly with the number of workers. Thus central parameter server does not often scale well with number with worker nor with depth of neural networks without proper balanced design.

%% One alleviation to the scaling problem in central parameter servers is to shard it. While there can be many physical sharding strategies, we focus our discussion to naive, ring and tree sharding. 

%% In naive sharing, a central parameter server is partitioned into physically disjoint parts, each serving a subset of keys in the parameter space independently. This is logically equivalent to a more powerful central parameter server with multiple interfaces and achieves the same optimality in terms of messages sent, communication latency and data movement per batch. Naive sharing however requires additional hardware resources and is more subject to delays in the network and stragglers in the parameter server shards. Similar to central parameter server, naive sharding requires linearly more hardware resources to scale system throughput with the number of workers.


%% A sharded parameter server can be logically organized as a ring, where each shard usually colocates with a worker. Gradients of each key are passed along the ring, performing aggregation with the gradient of the key on the current hop of the ring, and passing the aggregated buffer down the ring. A ring sharded parameter server trades communication latency for computation and smaller bandwidth requirement, because aggregation is distributed at each hop and only the aggregated buffer is sent out. Ring parameter servers cost $2N$ messages per key per batch, and a total data movement of $2NW$, but has latency of $2NT$. Ring parameter server removes the need for dedicated server hardware, but its latency (O($N$))scales linearly with the number of workers, which can be very harmful to the system throughput, especially for smaller neural networks. Ring parameter servers are generally not used in practice.

%% Another option is a reduction tree of parameter server shards. In this setup, a parameter server shard (which is a tree node) aggregates the gradients from all its children, and passes the aggregated buffer up the tree. The root then contains the final result. A reduction tree has the same merit of reduced bandwidth usage but significant reduced latency of $O(logN)$ at the cost of additional messages and more total data movement: In the special case of fan out 2, each key requires $4N$ messages per batch, with a latency of $2logNT$ and the total data movement is $4NW$. However, a reduction tree requires a special physical network layout to be implemented efficiently.



%% \subsection{Sharding and Colocation}
%% We have described the PHub as a centralized parameter server running on dedicated hardware. If a single PHub does not provide enough throughput, it may be scaled by sharding the model amongst multiple PHubs, still running on dedicated hardware.

%% Another common point in the design space is to colocate parameter server shards with workers. This increases the per-machine bandwidth requirement:
%% A sharded, non-colocated design with $N$ workers and a model size of $W$ requires each worker process to send $NW$ bytes, and each shard

%%  to send messages sent to $2N$ per key per batch (N push messages and N response messages) and has a total data movement of $2NW$. If enough bandwidth is 
%% One commonly-used trick to reduce total data movement in sharded parameter servers is to colocate servers and workers. For example, in naive sharding with colocation, a worker does not need to send keys processed by the local server shard through the network, saving a total of $1/N$ amount of data movement if each server is sharded with a worker.

%% However, modern training frameworks overlap computation of backward pass with synchronization, and this means that the parameter server process and the worker training process will contend for computation as well as communication resources, thus if caution is not taken, the benefit gain from reduced data movement due to colocation will not compensate for the loss of performance due to contention. Consider a shared network interface, with colocation on, the total data transmitted from the single node would be $4W(1-\frac{1}{N})$, versus $2W$ when colocation is off. This near $2x$ data movement for the node is detrimental to training performance.




==> SOCC 18/DesignSpace.tex <==
\section{\phub Design}
\label{sec:design}
%% Petuum/Poseidon
Based on \mysection\ref{sec:cloudTraining} findings, we propose a rack-scale PS, \phub, that reduces framework overhead with software optimizations, mitigates bandwidth insufficiency with a re-architected, balanced server configuration, and lowers network environment-induced overhead with topology-aware reduction algorithms. With \phub, we aim to:

% we rearchitected the PS to optimize the network stack, provide efficient gradient aggregation and optimization, and streamline the approach to sending and receiving gradients and model parameters. We also designed \phub to be a rack-scale parameter service, which allows job sharing and topology-aware reduction algorithms.

\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
\item Minimize gradient/model communication overhead.
%\item Gradient data should be laid out to exploit locality and enable overlap.
%\item Preserve locality and enable overlap of gradient processing and receiving.
\item Enable efficient gradient processing and overlapping with communication.
\item Balance communication and computation capabilities, both within and PS and between workers and the PS.
\item Allow low interference of co-running jobs and minimized cross-rack traffic.
\end{enumerate}

%\begin{table*}[t!]
%	\centering
%	\small
%	\begin{tabularx}{\textwidth}{|c|c|c|c||X|}
%		\hline
%		\phub   & \mxnet & Caffe2 & TensorFlow & Description\\
%		\hline
%		PHub::CreateService    & -   & -   & - & Find devices and creates a namespace.   \\
%		\hline
%		PHub::ConnectService & Van::Connect   &  Context::connectFullMesh  &   GrpcServer::Init  &  Rendezvous servers and workers. Exchanges addresses and queue pairs.  \\
%		\hline
%		PHub::InitService & KVStoreDistServer:: & AllReduceOp::Initialize & GrpcServer::Init & Allocates and registers  \\
%		                  & DataHandleEx        &     &     &   receive buffers.  \\
%		\hline 
%		PHub::PushPull   & KVStoreDist::PushImpl  & Algorithm::Run   & GraphMgr::SendInputs    &  Pushes the current gradients and pulls the update.  \\
%		                 & KVStoreDist::PullImpl  &                  & GraphMgr::RecvOutputs    &       \\
%		\hline
%		
%		\hline
%	\end{tabularx}
%	\caption{The Service APIs let PHub interface with multiple DNN training frameworks.}
%	\label{table:api}
%\end{table*}

\subsection{The \phub Service API and Interoperability with other Frameworks}
\phub{}'s API is designed for compatibility with multiple DNN training frameworks. Workers use \phub by first calling \code{PHub::CreateService} on the connection manager. This sets up access control and a namespace for the training job and returns a handle. The client side uses the handle to finish setup. \phub uses the namespace and an associated nonce for isolation and access control. 

Jobs call \code{PHub::ConnectService} to rendezvous servers and workers, exchanging addresses for communication. This call replaces \code{Van::Connect} in \mxnet, \code{Context::connectFullMesh} in Caffe2 and \code{GrpcServer::Init} in TensorFlow. \code{PHub::InitService} causes the current \phub instance to allocate and register receive and merge buffers. \phub also authenticates each worker's identity using the nonce. Authentication is a one-time overhead and once a connection is established, \phub assumes the remote identity associated with that address/port/queue number does not change during training.

\phub{}'s functional APIs include standard synchronous or asynchronous \code{PHub::Push/Pull} operations that are used in TensorFlow (\code{GraphMgr::SendInputs/RecvOutputs}) and \mxnet (\code{KVStoreDist::PushImpl/PullImpl}). \phub also includes a fused \code{PHub::PushPull} operation that perform a push, waits until all pushes are complete, and pulls the latest model. The fused operation often saves a network round-trip as push and pulls are frequently issued consecutively. This operator can serve as a drop-in replacement for Caffe2's \code{Algorithm::Run}.

\subsection{\phub Software Optimizations}
\label{sec:commonOptimizations}
This section describes software optimizations that benefit different stages in DDNN training across all common PS configurations. % the network stack optimization, gradient aggregation and optimization, fine-grained key chunking, and chunk-to-core mapping. These software optimizations benefit common PS setups.

\subsubsection{Network Stack Optimizations}
\label{sec:IBOptimization}
%We sought a solution that enabled zero-copy and kernel bypass for minimal latency and overhead when moving data.  
We sought to mitigate data movement latency with zero-copy and kernel bypass. We chose InfiniBand (IB) since we were already familiar with the Verbs API, and it is available in major cloud providers~\cite{AzureWin5:online}. Note that similar results could be achieved over Ethernet using RoCE, DPDK or other frameworks. We followed the guidelines from~\cite{rdma}; we tried two and one-sided RDMA, and two-sided send/receive operations and found similar performance in our workload. We briefly highlight some implementation details:

\noindent \textbf{Minimal Copy:} Leveraging InfiniBand's zero-copy capability, the only required data copy is between the GPU and main memory. When one GPU is used, this can be eliminated with GPU-Direct RDMA on supported devices.

\noindent \textbf{NUMA-Aware, One-shot Memory Region Registration:} Since a worker can operate on only one model update at a time, it is sufficient to allocate one read buffer (for the current model) and one write buffer (for update reception) for the model. To minimize InfiniBand cache misses, \phub preallocates all buffers in the NUMA domain where the card resides as a contiguous block.

\noindent \textbf{Minimal Metadata:} To maximize bandwidth utilization and minimize parsing overhead, \phub encodes metadata (such as callback ID and message opcode) into InfiniBand's queue pair number and immediate field. This saves \phub an additional PCIe round trip (from IB send scatter/gather) to gather metadata when sending messages.

%\phub leverages InfiniBand's zero-copy ability to reduce copies from the network to  GPU memory by re a per-key aggregation buffer set up during \code{Initialize}; the buffer aggregates gradients from multiple devices before pushing them out to the network. Thus, the only remaining copy to the buffer is from the GPU. For a single GPU, this copy can be eliminated using  GPU-Direct RDMA on supported devices. Before \phub uses InfiniBand as its data plane, it must register all memory used for communication. A worker can have only one model update executing concurrently. Thus, it is sufficient to allocate and register a buffer per worker for gradient reception, and a single buffer for the model. To minimize InfiniBand card memory registration cache misses, \phub pre-allocates all buffers to a single contiguous memory region that it registers. \phub memory registration is NUMA-aware. Memory is allocated on the same NUMA domain where the card resides to reduce QPI traffic between sockets. To keep track of pending operations, some metadata is required, such as current message meaning, sender and receiver information, opcode, and a timestamp used to execute the proper callback. To maximize bandwidth utilization, we encode all metadata into InfiniBand's queue pair number or immediate field. We also designed timestamps to be logical and deterministic, so they can be calculated by combining a global batch number with  message's key. This saves us an additional PCIe round trip (from IB send scatter/gather) to gather metadata when sending messages. 

\subsubsection{Gradient Aggregation and Optimization}
\label{sec:tallvswide}
Gradient aggregation and optimization are element-wise operations. Aggregation sums gradients for the same key from all workers. Optimization updates the model using aggregated gradients with an algorithm such as SGD. Our design goal is to overlap aggregation and optimization of different keys with communication.

% for 2690v4: AVX max speed is 2.1 GHz, 1 256-bit add per cycle (2 if FMA multiplying by 1, but that's annoying)
% so 2.1 GHz * 8-float vectors (32 bits) * (2 reads + 1 write) * 28 cores
% so 470 billion ops/second, 5645 GB/s bidir for 2 read 1 write, 1882 GB/s if aggregation buffers (1read, 1write) are in cache
%% Gradient aggregation could be performed on the CPU or GPU. Here, we posit that the CPU is sufficient for this job.
%% Aggregation is simply vector addition: we read two floats and write one back.
%% For modern CPUs, this is fast: if we keep the processors' AVX ALUs fed, we can perform 470 single-precision giga-adds per second, requiring 5.6TB/s of load/store bandwidth.
%% A typical dual socket server can sustain up to 140GB/s memory bandwidth. 5.6TB/s is impractical for the large vectors involved in DNN training workloads, making aggregation inherently memory bound. There is thus little point in copying gradients to GPU to perform aggregation.
Gradient aggregation could occur in the CPU or GPU~\cite{GeePS}. Here, we posit that the CPU is sufficient for this job.
Aggregation is simply vector addition: we read two floats and write one back.
%Our evaluation hardware is typical of modern dual socket servers. 
With our typical modern dual socket server, if we keep our processors' AVX ALUs fed, we can perform 470 single-precision giga-adds per second, requiring 5.6 TB/s of load/store bandwidth.
But the processors can sustain only 120 GB/s of DRAM bandwidth. 5.6 TB/s is impractical %for the large vectors found 
in DNN training workloads, making aggregation inherently memory bound. Thus, copying gradients to a GPU for aggregation is not helpful.

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=5 5 15 5,clip]{Figures/AggregationExperiments.pdf}
	\caption{Ways of gradient aggregation. A thread (arrow) aggregates over the array (gray rectangle) of gradients from a worker. }
	\label{fig:gradientAggregation}
\end{figure}


There are many ways to organize threads to perform aggregation.
%We start with the case where all workers' gradient arrays for a given key are received. 
Figure \ref{fig:gradientAggregation} shows four options we prototyped， assuming gradient arrays are available at once. We found that the best performance was achieved using the two discussed below; other schemes suffered from too much synchronization overhead, poor locality and/or high latency.

\textit{Wide aggregation} is typical to systems like \mxnet that call BLAS routines for linear algebra. In these systems, a group of aggregation threads process one gradient array at a time; each thread works on a partition of that array. 
%When the current array is done, the group moves to the next.

A variation of wide aggregation is \textit{tall aggregation}, which chunks a gradient array into mini-chunks of predefined sizes; each thread works independently to process the same chunk across all gradient arrays for a given key. This is the preferable way to organize threads for many reasons.
First, gradient arrays do not arrive instantly. For a large key (e.g., a fully connected layer), aggregation and optimization cannot start for wide aggregation until the key is fully received; for tall aggregation, the process can start as soon as the first chunk is received.
Second, in wide aggregation, it is challenging to balance the number of threads dedicated to aggregation and to optimization, let alone partitioning threads to work on different keys since they can arrive at the same time; %, as the optimal assignment can be DNN dependent; 
thread assignment for tall aggregation is natural.
Third, wide aggregation induces queuing delays: it effectively processes one key at a time versus tall aggregation's many ``mini-queues.''
Fourth, wide aggregation puts many threads to work in lock-step on pieces of data, which incurs non-trivial synchronization overhead; tall aggregation requires no coordination of threads as aggregation is an element-wise operation.

%and tall aggregation allows aggregation to start as soon as a chunk is received, without waiting for the entire gradient array to arrive (some networks have large fully connected layers of size up to tens of megabytes), overlapping communication and computation. More importantly, it is challenging to balance the number of threads that are dedicated to aggregation and optimization if they overlap. 

%Tall aggregation essentially creates many mini queues, alleviating queueing delays. Wide aggregation approach on the other hand, can incur high overhead from repeated thread coordination, and working on only one gradient (which belongs to the same key) at a time effectively forms a queue causing delays. Furthermore, the optimal value for number of threads is workload dependent in wide aggregation. Figure \ref{fig:tallVSWide} compares these two approaches. We chose tall aggregation in \phub.

\phub tracks the number of currently aggregated mini-chunks for a given key. When a chunk is received from all workers, it can be optimized. This step is natural in \phub: the thread that aggregates a particular chunk also optimizes that chunk. As a result, \phub{}'s aggregation and optimization scheme effectively maps a particular chunk to a single core (since \phub pins threads to cores). On the other hand, \mxnet uses wide optimization: when a key is fully aggregated, another set of threads is launched to perform aggregation. No overlap occurs between key aggregation and optimization. 
%% \phub tracks the number of currently aggregated chunks for a given key.
%% \phub counts the number of workers for which it has aggregated a chunk.
%% When a chunk has been received from all workers, it can be optimized.
%% This step is natural in \phub: the thread that aggregates a particular chunk also performs optimization for that chunk.
%% As a result, \phub{}'s aggregation and optimization scheme effectively maps a particular chunk to a single core.
%% Conversely, \mxnet uses wide optimization: when a key is fully aggregated, a new set of parallel tasks is launched to perform optimization.
%% No overlap occurs between the two steps. Figure \ref{fig:tallVSWide} compares throughput of tall and wide aggregation in \phub and \mxnet: tall aggregation/optimization outperforms their wide counterparts.


%Similar to gradient aggregation, optimizer is another element-wise step. \phub naturally assign optimization task of each mini chunk of a key to the core that is responsible for its aggregation (tall optimization). This allows optimization and aggregation of a same key to overlap\footnote{As a side note, \mxnet uses wide optimization as well. When a key is fully aggregated, it moves to the optimization stage and potentially another group of threads is launched. There is no overlapping between key aggregation and optimization.}.

%% We implemented two variants of each optimizer: one that uses normal cached loads and stores, and one that bypasses the caches with non-temporal prefetches and stores. This allowed us to test whether caching only the model or gradients wold provide a benefit. We found the temporal version to be more effective. \phub{}'s aggregators and optimizers are fully extensible: implementations that comply with \phub{}'s API can be used during runtime.

We explored the benefits of caching by implementing two variants of each aggregator and optimizer: one using normal cached loads and stores, and one with non-temporal prefetches and stores. We found it beneficial to cache both the model and gradients. \phub{}'s aggregators and optimizers are fully extensible: implementations that comply with \phub{}'s API can be used during runtime.

\subsubsection{Fine-grained Key Chunking}
%\phub chunks key for two purposes. First, fine-grained key chunking lets \phub balance server and processor core load. This is important because different neural network layers can have significantly different total weight sizes, from a few bytes to tens of MBs. Second, fine-grained key chunking supports tall aggregation and optimization, so processor cores can be fully utilized.

%This makes balancing server and processor core load challenging. By chunking the weight size into a series of virtual layers (a set of virtual keys) of small, fixed size, \phub can balance load of processor cores optimally.These virtual keys are then treated independently in model update; \phub relies on fined grained key chunking to support tall aggregation and optimization, usually at the size of a few to tens of kilobytes.

Chunking in \phub differs from chunking in other systems in key ways. Initially, our goal is to balance load at a fine-grained level across cores and interfaces rather than across server shards: chunking is turned on even when a centralized PS is used. Next, we would expect our optimal chunk size to be the nearest, smallest message size that can saturate network bandwidth, whereas systems like \mxnet prefer larger key chunk sizes to avoid excessive thread synchronization overhead.
%In fact, \phub defaults to 32KB of chunk, while \mxnet defaults to a 4MB chunk size.
In fact, \phub's default is 32KB, while \mxnet's is 4MB.
Finally, key chunking enables another important optimization: the overlapping of gradient transmission with aggregation and optimization. Aggregation starts only after a key's entire gradient array is received; and for large layers, this adds significant delay. With small key chunks, \phub enables ``streaming'' aggregation and optimization.

\begin{figure}[t!]
	\centering
	\includegraphics[width=.8\linewidth,trim=1 0 1 1,clip]{Figures/MappingChunkToCore.pdf}
	\caption{The process of mapping a chunk to a core in \phub using fine grained key chunking. Keys are chunked into virtual keys. The highlighted key is delivered to a highlighted (fixed) core through a highlighted (fixed) queue pair and completion queue. }
	\label{fig:mappingChunkToCore}
\end{figure}


\subsubsection{Mapping a Chunk to a Core}
\label{sec:chunk2core}
\phub's assignment of chunks to cores is computed during initialization. At that time, the set of all keys is sharded across the cores and interfaces available on PS nodes.
A specific chunk is always directed to a particular queue pair,
which is associated with a shared completion queue on the chunk's core.
%the responsible core has a single completion queue for all its associated queue paris.
%which is associated with a completion queue and is eventually processed by that single core.
All message transmission, reception, and processing for that chunk is done on that core. Cores do not synchronize with each other. Once processed, a chunk is transmitted back to the workers on its originating path. The worker side of \phub assembles and disassembles a key, a process that is transparent to the framework.

\phub{}'s chunk assignment scheme provides significant locality benefits. The same key likely arrives around the same time from multiple workers; the associated aggregation buffer is reused during this period. The scheme also encourages locality in the InfiniBand interface in the queue pair and memory registration caches, which can further benefit performance.

This scheme imposes challenges in balancing load across cores, queue pairs and completion queues. \phub uses a 4/3 approximation set partition algorithm to balance each component's workload at each level, which produces practically balanced assignments in our experiments.





==> SOCC 18/Discussions.tex <==
\section{Additional Related Work}
\label{sec:discussion}

This section augments the related work discussed in \mysection\ref{sec:background}.

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=8 4 4 2,clip]{Figures/VSGloo.pdf}
	\caption{Left: Comparing Caffe2 + Gloo and \mxnet + \phubbox on an 10Gbps InfiniBand network. Right: Comparing \mxnet + Gloo and \mxnet + \phubbox on a 56Gbps InfiniBand network with \code{ZeroComputeEngine}. }
	\label{fig:gloo}
\end{figure}

\vspace{0.05in}
\noindent \textbf{Other Communication Schemes:}
%\subsection{Other Communication Schemes}
Parameter servers are not the only way to perform model updates. Frameworks such as CNTK and Caffe2 can use HPC-like approaches, such as collective communication operations~\cite{Thakur:2005:OCC:2747766.2747771, firecaffe}.

To understand how \phub compares to other communication schemes, we first ran Caffe2 and \mxnet with \phubbox on a cloud-like network. We used InfiniBand for both systems. We evaluated the fastest algorithm in Gloo: recursive halving and doubling, used in \cite{ImageNetIn1Hour}. Figure \ref{fig:gloo} (left) shows the result: \phubbox was nearly 2x faster. 
%This is expected because collectives, like colocated servers, cause roughly 2x traffic per link in the system, bottlenecking training performance in network bound environment.

We ported Gloo to \mxnet to better asses both systems. Gloo implements blocking collective operations, but \mxnet expects non-blocking operations. Therefore, we measured an optimistic upper bound by letting Gloo start aggregating the entire model as soon as the backward pass started, as if all gradients were available instantaneously. Since Gloo only does reduction, we ran our SGD/Nesterov optimizer on all nodes after reduction was complete. We used 56 Gbps IB and \code{ZeroComputeEngine} to remove network and worker bottlenecks. Figure \ref{fig:gloo} (right) shows the result; %when given an infinitely fast compute engine and ample communication resources, 
\phubbox sustained higher throughput and provided better scaling up to its limit. Two reasons account for this difference. First, collectives suffer from the same problem as colocated PSs: the interface on each participating node must process nearly 2x the data (Gloo's \code{allreduce} starts with a \code{reduce-scatter} followed by an \code{allgather}~\cite{Thakur:2005:OCC:2747766.2747771}). 
% illustrates the complexity of the scheme). 
Second, collectives frequently use multi-round communication schemes %uses multiple rounds of communication to perform reduction: 
($logN$ rounds for $N$ workers in this case), whereas \phubbox uses only 1 round. %, minimizing reduction latency.

% third,  \phubbox moves the minimum amount of data in the network: $2MN$, where $M$ is the model size, and halving and doubling moves 

\vspace{0.05in}
\noindent \textbf{Compression, Quantization, Sparse Vector Communication, and Other Mechanism for Traffic Reduction:}
Orthogonal to our work are techniques to reduce gradient traffic. These techniques trade higher overhead in preparing and processing network data for lower network bandwidth usage. For example, \mxnet{} supports a 2-bit compression scheme, similar to \cite{cntk1bt}. We compared \phub running on \phubbox to \psliteib with 2-bit compression: \phubbox without compression still beat \psliteib by 2x. 

%To gauge how this work affects \phub, we emulated 1-bit SGD in an 8-worker throughput experiment by modifying our network layer to send and receive only the first $1/32$nd of the buffer; all buffer elements were processed by the worker and the server. We used \psliteib as a baseline due to ZMQ limitations and ran this experiment with VGG and \code{ZeroComputeEngine}. With normal 32-bit floats, \phubbox was 2.13x faster than normal sharded \psliteib; with our 1-bit SGD emulation, \phubbox provided a benefit of 1.5x over the modified baseline. Thus, while techniques like 1-bit SGD can change the compute-to-communication ratio, using \phub still offers a benefit.

Other examples include Sufficient Factor Broadcast (SFB) \cite{poseidon,DBLP:journals/corr/XieKX14}, which decomposes the gradient of a fully connected layer (FCL) into the outer product of two vectors. SFB uses a P2P broadcast scheme whose overhead scales quadratically with the number of machines, making it suboptimal for large scale training. Project Adam~\cite{projectAdam} sends activation and error gradient vectors for reconstruction on server. Both techniques have limited applicability as they only apply to FCLs, which are small or unused in recent neural networks~\cite{DBLP:journals/corr/SzegedyIV16,RESNET,inception-v3,ResNext}.
%either no longer exists \cite{DBLP:journals/corr/SzegedyIV16} or is insignificant in size when compared to the full model in more recent neural networks (e.g., \cite{RESNET,inception-v3,ResNext}).

\phub can also work with gradient compression \cite{DBLP:journals/corr/abs-1712-01887} to gain further benefits from its low latency communication stack, fast aggregation and optimization.

%% \vspace{0.05in}
%% \noindent \textbf{Other Synchronization Patterns:}
%% %Another recent line of work uses synchronization patterns other than those on which we focused.
%% Two examples include asynchronous updates~\cite{recht2011hogwild,projectAdam,googleDNN} and relaxed consistency~\cite{DBLP:journals/corr/DaiKWHGX14,SSP,BSP,184014,Wei:2015:MCC:2806777.2806778}. In both cases, there may be less opportunity to aggregate before updating the model, but \phub{}'s lower latency will still provide benefit. These patterns exceed our current scope.% of work.

%% Another technique, called sub-mini-batching \cite{subminibatching}, lets GPUs train batch sizes that do not fit in memory by partitioning each large mini-batch into sub-mini-batches. Statistically, this is equivalent to mini-batching. %because it requires the same number of parameter exchanges to achieve convergence.%
%% It does so by increasing the wall clock time spent in computation and thus reducing synchronization frequency, which ultimately \textit{increases} total training time. Sub-mini-batching is best solved by scaling out to more GPUs, where \phub can be of help.



==> SOCC 18/Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
We added support for \phub{}'s API to \mxnet, replacing its PS. We evaluated \phub by comparing it to \mxnet{}'s unmodified PS. We had four goals in our evaluation: (1) to assess the impact of \phub software and the \phubbox hardware on training throughput, (2) to identify the importance of each optimization, (3) to determine the limits of \phubbox, (4) to evaluate effectiveness of \phubbox as a rack-scale service. and (5) to demonstrate the cost-effectiveness of the \phub.
\subsection{Experimental Setup}
We evaluated our system with 8 worker nodes and one specially configured \phubbox node. The workers were dual socket Broadwell Xeon E5-2680 v4 systems 
% with 28 cores at 2.4 GHz -- we can omit details as product model implies clockspeed etc to save some space.
and 64 GB of memory using 8 dual-rank DDR-2400 DIMMs. Each worker had a GTX 1080 Ti GPU % with 11 GBs of memory 
and one Mellanox ConnectX-3 InfiniBand card with 56 Gbps bandwidth in the same NUMA domain. The \phubbox machine was a dual socket Broadwell Xeon E5-2690 v4 system with 28 cores % running at 2.6 GHz 
and 128 GBs of memory using 8 dual-rank DDR-2400 DIMMs. \phubbox had 10 Mellanox ConnectX-3 InfiniBand cards, with 5 connected to each socket. Hyperthreading was disabled. Machines were connected with a Mellanox SX6025 56 Gbps 36-port switch.

The machines ran CentOS 7.3 with CUDA 8 and CuDNN 7 installed. Our modifications to \mxnet and its PS (PS-Lite) were based on commit 2ce8b9a of the master branch in the PS-Lite repo. We built \mxnet with GCC 4.8 and configured it to use OpenBLAS and enable SSE, the Distributed Key Value Store, the \mxnet Profiler, and OpenMP. We used Jemalloc, as suggested by \mxnet.

\subsection{DNNs Used in the Evaluation}




We evaluated \phub{}'s performance by training state-of-the-art deep neural networks using reference code provided with \mxnet. %While we did not modify the code, 
%We adjusted layer count, per worker batch size, and the number of workers and servers to launch. 
We implemented cache-enabled SGD with Nesterov's accelerated gradient method \cite{nesterov1983method} and aggregator for \phub{}. We chose a per GPU batch size of 32 when possible; for ResNet 269 and ResNext 269, we used 16 and 8, respectively, since 32 did not fit in the GPU. We did not use MXNet's GPU memory optimizations~\cite{chen2016training} because they slow down training.

\begin{table}[t!]
	\centering
	\footnotesize
	\begin{tabular}{|c|c|c|c|}
		\hline 
		Name (Abbr)           & Model Size & Time/batch & Batch \\
		\hline
		AlexNet (AN)      & 194MB & 16ms &  32 \\
		\hline 
		VGG 11 (V11)       & 505MB & 121ms & 32 \\
		\hline
		VGG 19 (V19)      & 548MB & 268ms & 32 \\
		\hline
		GoogleNet (GN)   &  38MB & 100ms & 32 \\
		\hline
		Inception V3 (I3) & 91MB  & 225ms & 32 \\
		\hline
		ResNet 18 (RN18)   & 45MB & 54ms & 32 \\
		\hline
		ResNet 50 (RN50)   & 97MB & 161ms & 32 \\
		\hline  
		ResNet 269 (RN269)  & 390MB & 350ms & 16 \\
		\hline
		ResNext 269 (RX269) & 390MB & 386ms & 8 \\
		\hline
	\end{tabular}
	\caption{Neural networks used in our evaluation. Time/batch refers to the forward and backward compute times for a batch.}
	\label{table:networkCharacterization}
\end{table}


Table \ref{table:networkCharacterization} summarizes the neural networks used in our evaluation, which include both winners of the ImageNet challenge and other recent, popular networks. We used the reported model size from \mxnet and measured the forward and backward passes time on a single GPU. % with the batch sizes described previously. %We turned off aggregation and optimization for this measurement; therefore, the time represents only that for forward and backward passes.

We report only training throughput in our evaluation since our modifications did not change accuracy because they did not change computations that were performed. We trained multiple DNNs to convergence to verify this.



\subsection{Training Performance Evaluation}
%We explored training performance using \phub, normalized to unmodified \mxnet's performance. 
We include multiple results to highlight the effects of different software and hardware optimizations on \phub{}'s training performance. We measured training performance by comparing the total time of 200 iterations. We used two IB network configurations. This lets us compare training performance for two different compute/bandwidth ratios: (1) where GPUs were much faster than the network, and (2) with ample network bandwidth resources. In both setups, we used 8 workers.
%Both results reflect the benefit of an optimized gradient processing pipeline from the \phub software stack and the benefit of using hardware with balanced resources (\phubbox). %\TODO{DO WE NEED 56Gbps IT LOOKS BAD WITH NEW BASELINE.}

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=8 4 4 4,clip]{Figures/IBBenefits.pdf}
	\caption{Speedup from a faster data plane that supports zero copy.}
	\label{fig:IBBenefits}
\end{figure}

\subsubsection{Benefit of a Faster Data Plane}
Figure \ref{fig:IBBenefits} shows the performance of replacing the communication stack of the \mxnet PS with a native InfiniBand implementation (\psliteib) that had all optimizations noted in \mysection\ref{sec:IBOptimization}. This lets us see the benefit of switching to an optimized network stack without changing the PS architecture. %We believe similar speedup can be observed on a RoCE-based implementation, because the benefit comes mainly from zero copy. 
We used our \textit{enhanced baseline \psliteib} in all the following evaluation.

\subsubsection{Other Software and Hardware Optimizations}
We now quantify further benefits from \phub{}'s software and hardware optimizations. 
We used CS \psliteib in this comparison.
\pshard{} results were obtained by running \phub software on each worker as CS PSs. \phubbox results represent running \phub software on our single \phubbox machine as a NCC PS. We omit results for NCS and CC PSs for clarity. They performed similarly to \phubbox results.




% placed here to be on same page as text
\begin{figure*}[t!]
	\includegraphics[width=\linewidth,trim=4 4 4 4,clip]{Figures/8GbpsRealTraining_SOCC.pdf}
	\caption{Training performance on a cloud-like 10 Gbps network. Results are normalized to sharded \psliteib (\textit{enhanced baseline}).}
	\label{fig:real-8gb}
\end{figure*}

% placed here to be on same page as text
\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=8 4 4 4,clip]{Figures/56GbpsRealTraining_SOCC.pdf}
	\caption{Training performance on a 56 Gbps network compared to \psliteib (\textit{enhanced baseline}). Computation speed bottlenecked training throughput for all but AlexNet and VGG.}
	\label{fig:real-56gb}
\end{figure}

\begin{figure}
	\includegraphics[width=\linewidth,trim=4 2 2 4,clip]{Figures/PHubOverheadBreakdown.pdf}
	\caption{Progressive overhead breakdown of \phub. Compared to Figure~\ref{fig:overheadBreakdown}, GPU compute time now dominates training time. Aggregator and optimizer have minimum overhead, and are barely visible.}
	\label{fig:phubOverheadBreakdown}
\end{figure}

Figure~\ref{fig:real-8gb} shows training performance on a cloud-like 10 Gbps network, obtained by down-clocking our IB links. In this configuration, the ratio of GPU batch execution time to network serialization delays is such that the reduced communication and faster aggregation of \phubbox significantly affects runtime. In addition, we provide speedup when training with only 7 workers and \phubbox, \textit{so that the total machine count in the system is equal to the baseline}.

Figure~\ref{fig:real-56gb} shows training performance on 56 Gbps InfiniBand.
%% In this setup, training throughput of networks such as GoogleNet, Inception, ResNet, and ResNext is limited by speed of forward and backward passes, the time to execute forward and backward passes exceeds that of parameter exchange; thus, raising network bandwidth only marginally affects the total throughput of \phub versus \psliteib.
In this setup, for networks such as GoogleNet, Inception, ResNet, and ResNext, forward and backward pass execution time limits training throughput; thus, raising network bandwidth only marginally affects the total throughput of \phubbox versus \psliteib. Since \phub never slows down training, we omit results of these networks (1x speedup) for clarity. We expect larger speedups with newer, faster GPUs, such as the NVidia V100 for these networks. Significant speedup is still achieved with models that have large communication-to-computation ratios, such as AlexNet and VGG; these models remained network-bound even on 56 Gbps links.

%In both cases, the gap between \phubbox and \pshard highlights the benefits of non-colocated servers: \textit{they roughly halve the per link bandwidth usage, which makes a significant performance difference in the cloud}. 
The gap between \pshard and \psliteib signifies the benefit of software optimizations in \mysection\ref{sec:tallvswide}-\mysection\ref{sec:phub}, while the gap between \pshard and \phubbox highlights the benefit of both a non-colocated server that \textit{halve the per link bandwidth usage, which made a significant performance difference}, and the optimizations in \mysection\ref{sec:phub}.

%The gap between \pshard and \psliteib shows the benefit of \phub software stack optimizations (\mysection\ref{sec:commonOptimizations}), and the gap between \psliteib and the baseline reflects the effectiveness of an optimized communication stack (\mysection\ref{sec:IBOptimization}). %\TODO{more explanation}

%Figure~\ref{fig:real-2gb} shows an unbalanced condition where the provisioned compute resource is significantly faster than network bandwidth. We achieved this by reducing our network bandwidth to 2 Gbps; this lets us model the performance of 28x faster GPUs with our 56 Gbps network. Although the baseline parameter servers are more than capable of processing messages at this network speed, the workers' network bandwidth is highly contended by its colocated parameter server instance during parameter synchronization. \phub achieves up to 3x speedup over sharded PSLite-ZMQ by avoiding this worker/shard contention, and providing faster aggregation and optimization.

Figure \ref{fig:phubOverheadBreakdown} breaks down the overhead in different distributed training stages when running \phub in the same setup as Figure \ref{fig:overheadBreakdown}. Compared to Figure \ref{fig:overheadBreakdown}, \textit{\phub reduces overheads from data copy, aggregation, optimization, and synchronization and fully overlaps these stages, shifting the training back to a compute-bound workload.}


\subsection{Performance with Infinitely Fast Compute}
We used a benchmark to assess the efficiency of \phub{}'s gradient processing pipeline to avoid being bottlenecked by our workers' GPUs. We implemented a special \mxnet engine, called \code{ZeroComputeEngine}, based on the original \code{ThreadedEnginePerDevice}, which replaces training operators (such as convolution) with an empty routine. Only the synchronization operators (\code{WaitForVar}, \code{KVStoreDistPush} and \code{KVStoreDistPull}) are actually executed. This engine effectively simulates arbitrarily fast forward and backward passes on the worker side, pushing the limits of \phub.

We used ResNet 18 as the test network. We first measured how fast each worker can run in this setup by running a single worker with the \phubbox, then gradually added more workers to plot total system throughput.

%By spreading the communication equally on the 10 interfaces on the \phubbox and utilizing all processors, a worker can perform 110 iterations per second, producing 10GB/s of bidirectional throughput. A single \phub core is enough to saturate a worker. Aggregation and optimization are disabled for this benchmark. We set our "training batch size" to 1 for this benchmark so we measure only the parameter exchange rate. 

Figure \ref{fig:FakeTrainingWithAggOpt} shows the results of running the benchmark with \phubbox, \pshard and multiple baseline configurations. \phubbox  provided linear scaling with 8 workers and outperformed the baseline by a large margin (up to 40x). \phubbox had 2x the speedup of \pshard{} because each of its interface needed to move only about half the amount of data compared to colocated servers.

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=1 1 1 1,clip]{Figures/FakeTrainingWithAggOpt.pdf}
	\caption{\phubbox provides linear scaling of throughput for 8 worker nodes with infinitely fast compute, training ResNet 18.}
	\label{fig:FakeTrainingWithAggOpt}
\end{figure}


\subsection{Exploiting Locality}
\label{sec:locality}
To postpone hitting the memory bandwidth limit, it is crucial to exploit locality in network interfaces and processor caches. This section evaluates the effectiveness of \phub{}'s key assignment scheme and tall aggregation/optimization in leveraging locality.

\vspace{0.05in}
\noindent \textbf{Key Affinity in \phubbox:}
%\subsubsection{Key affinity in \phubbox}
\label{sec:affinity}
We evaluate two schemes for connecting workers to \phubbox to exploit locality and load balancing. In \textit{Key by Interface/Core mode}, workers partition their keys equally across different interfaces on the \phubbox. This mode better utilizes cache by binding a key to a particular interface, core and a NUMA node. %, computation for that key can more effectively use cache. 
This mode also exploits locality in time as workers are likely to generate the same key close to each other in synchronous training.

In \textit{Worker by Interface mode}, each worker communicates with the server through a single interface. This lets \phub exploit locality within a single worker. It also provides naturally perfect load balancing across interfaces and cores at the cost of additional communication and synchronization for each key within the server because keys are scattered across all interfaces and sockets.

%We used the same \code{ZeroComputeEngine} to evaluate the aforementioned approaches. 
We found that Key by Interface/Core provided 1.43x (790 vs 552 exchanges/s) better performance than Worker by Interface mode with \code{ZeroComputeEngine}. The locality within each worker could not compensate for synchronization and memory movement costs.


\vspace{0.05in}
\noindent \textbf{Tall vs. Wide Parallelism:}
%\subsubsection{Tall vs. Wide Aggregation and Optimization}
%Figure \ref{fig:tallVSWide} compares throughput of \phub's tall approach to aggregation and optimization with \mxnet's wide approach. 
We evaluated tall aggregation vs \mxnet{}'s wide approach with ResNet 50. Tall outperformed wide by 20x in terms of performance  and provides near-perfect scaling to multiple cores. Tall aggregation benefited from increased overlap compared to wide, and wide was further hurt by the cost of synchronization.

%\begin{figure}[t!]
%	\includegraphics[width=\linewidth,trim=3 1 2 3,clip]{Figures/TallVSWide.pdf}
%	\caption{Tall aggregation/optimization was more efficient than wide aggregation/optimization.}
%	\label{fig:tallVSWide}
%\end{figure}

\vspace{0.05in}
\noindent \textbf{Caching Effectiveness in \phub:}
%\subsubsection{Caching effectiveness in \phub}
\label{eval:cache}
Caching benefits many \phub operations. For example, models can be sent directly from cache after being updated, and aggregation buffers can reside in cache near the cores doing aggregation for those keys. We now evaluate the effectiveness of caching in \phub by measuring memory bandwidth usage.

\begin{table}[t!]
	\centering
	\footnotesize
	\begin{tabular}{|c|c|c|}
		\hline 
		& Mem BW & Throughput\\
		\hline
		Opt/Agg Off & 77.5 & 72.08 \\
		\hline 
		Caching Opt/Agg & 83.5 & 71.6 \\
		\hline
		Cache-bypassed Opt/Agg & 119.7 & 40.48 \\
		\hline
	\end{tabular}
	\caption{Bidirectional memory bandwidth (GB/s) utilization in \phub when training VGG with 8 workers. The maximum memory bandwidth for the machine is 137 GB/s for read-only workloads and 120 GB/s for 1:1 read:write workloads as measured by LikWid and Intel MLC.}
	\label{table:cacheUtilizationAndAggregationOverhead}
\end{table}

Table \ref{table:cacheUtilizationAndAggregationOverhead} shows the memory bandwidth costs of communication, aggregation, and optimization on \phubbox. We used 8 workers running a communication-only benchmark based on the VGG network, chosen because it had the largest model size. We first ran the benchmark with no aggregation or optimization, and we then added our two aggregation and optimization implementations.

Without aggregation and optimization, \phubbox{}'s bidirectional memory bandwidth usage was stable at 77.5 GB/s. No cache was used in this case because \phubbox did not touch the data (only the network interface did).

We found that the caching version of the aggregator and optimizer performed significantly better than the cache-bypassing version, which hit the maximum memory bandwidth available on the \phub machine when combined with the memory bandwidth of worker sends and receives. The caching version, on the other hand, added only 8\% to total memory bandwidth usage; aggregation and optimization added only 1\% of overhead to the overall throughput in this benchmark, fully overlapping gradient transfer. 

%One interesting point here is that only a fraction of the cores are required to saturate the memory bandwidth when doing aggregation and optimization. Our experiments showed that 4 cores per socket are sufficient to saturate bandwidth for these processors, but to avoid synchronization overhead in the network layer we use one core per interface (5 per socket; 10 total) for the rest of our evaluation.

%We now compare \phub's aggregator and optimizer performance with our baselines using a synthetic benchmark no-computation benchmark based on ResNet-18. Here, we add an additional baseline using MXNet with an allreduce implementation from the Gloo~\cite{Gloo,ImageNetIn1Hour} collectives library. 

%Gloo implements blocking collective operations, but \mxnet expects non-blocking operations, so we provide an optimistic upper bound on aggregation performance with Gloo by allowing it to start aggregating the entire model as soon as the backward pass starts, as if the entire gradient is available instantaneously. We evaluate the two fastest algorithms in Gloo: recursive halving and doubling, which is used in \cite{ImageNetIn1Hour}, and chunked ring, which has low analytical complexity and is empirically fast in our measurement. Since Gloo only does reduction, we run our SGD/Nesterov optimizer on all nodes after reduction is complete. We include only a colocated configurations for the sharded baselines in this experiment.

%Figure \ref{fig:cacheUtilizationAndAggregationOverhead} shows the result. \phub beats sharded PSLite-ZMQ and PSLite-IB 7.6x and 3.9x, respectively,  demonstrating the efficient implementation aggregation and optimization in \phub.  \phub also beats Gloo's chunked ring and halving and doubling algorithms by 4.7x and 6.3x, respectively. This is expected since the \phub uses a single round of communication per key, per iteration, whereas for our 8 workers the collective algorithms use 7 and 3 rounds, respectively, and bandwidth is not a bottleneck in this test. We repeated this under a bandwidth limited environment (2Gbps), and found our speedup over these two collectives algorithms is 1.9x and 2.9x. In~\cite{ImageNetIn1Hour}, the halving and doubling algorithm was faster than the chunked ring, but we see the opposite result; we believe this is due to the higher implementation complexity of halving and doubling, and the lower number of workers in our cluster---too few to see the asymptotic complexity benefit. 

%Finally, \phub has a 2x advantage over PShard, which again is limited by network bandwidth due to colocation.


\subsection{Tradeoffs in Fine-Grained Key Chunking}
\label{sec:commParam}
We now examine tradeoffs in the communication layer concerning the size of key chunks and queue pair counts.

\begin{figure}[t!]
	\includegraphics[width=\columnwidth,trim=4 8 2 4,clip,]{Figures/QPandKeyChunkSize.pdf}
	\caption{Effect of chunk size and queue pair count on throughput.}
	\label{fig:QPandKeyChunk}
\end{figure}

\vspace{0.05in}
\noindent \textbf{Size of key chunks:}
%\subsubsection{Size of key chunks}
\label{sec:keyChunking}
\phub leverages fine-grained key chunking to better balance load and overlap gradient reception and aggregation. Figure \ref{fig:QPandKeyChunk} (left) evaluates the effect of chunk size with \code{ZeroComputeEngine} on \phubbox. Larger chunk sizes improved network utilization, while smaller sizes improved overlapping. We found 32KB chunk size to be optimum: this is likely due to our interfaces' maximum injection rate and aggregation pipeline latency.

\vspace{0.05in}
\noindent \textbf{Queue Pair Count:}
%\subsubsection{Queue Pair Count}
%\phub uses queue pairs to direct keys to cores. The card manages queue pairs; hence, 
A worker needs at least one queue pair per interface with which it communicates. Queue pairs have state, which is cached on the card. When that cache misses frequently, communication slows. For \phubbox to use 10 interfaces, we need a minimum of 10 queue pairs per worker. More queue pairs could enable concurrent transmission from the same worker and reduce head of line blocking, but it increases the queue pair cache miss rate. Figure \ref{fig:QPandKeyChunk} (right) evaluates the tradeoff, showing that fewer queue pairs was optimal.


\subsection{Limits on Scalability}
\label{sec:scability} 
The scalability of \phub is inherently limited by available total memory, network or PCIe bandwidth. This section explores how close \phub gets to these limits. We use \phubbox to answer these questions. \phubbox achieves a 1:1 read:write memory bandwidth of 120 GB/s and a bidirectional network bandwidth of 140 GB/s. To determine how much bandwidth can be utilized,
%we configured varying numbers of worker machines running \code{ib\_write\_bw},
we added an additional IB interface to each of our 8 machines to emulate 16 workers and configured varying numbers of emulated workers running \code{ib\_write\_bw},
%, and configured varying numbers of worker machines running \code{ib\_write\_bw},
each with 10 QP connections to the \code{ib\_write\_bw} process on \phubbox. These pairs of processes did repeated RDMA-writes to two 1 MB buffers on the other side. We set the PCIe read request size to 512 bytes. This configuration was chosen to mirror the setup of an actual training system while maximizing total system throughput. 
%We used \code{likwid} to measure the maximum system throughput in terms of memory bandwidth. 

To our surprise, we found that the peak memory bandwidth usage never exceeded more than 90 GB/s, far from the limit of both the aggregate network card and memory. This suggests that the bottleneck lies somewhere else. 

We then built a loopback microbenchmark that used the IB cards to copy data locally between RDMA buffers. This isolated the system from network bottlenecks and involved only the NIC's DMA controllers and the processor's PCIe-to-memory-system bridge. This microbenchmark also achieved only 90 GB/s. Based on this experiment, we believe that \textit{the limit of throughput in our current \phub system is the PCIe-to-memory-system bridge.}

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=2 2 2 2,clip]{Figures/Scalability.pdf}
	\caption{\phubbox{} scalability is limited by the throughput of the PCIe to the on-chip network bridge of the PBox processors. \phub{} can utilize 97\% of the measured peak PCIe bandwidth.}
	\label{fig:scalablity}
\end{figure}

Figure \ref{fig:scalablity} summarizes this experiment. The InfiniBand/PCIe limit line shows an ideal case where unlimited cache line transfers can be performed. However, this rate was not achievable even with a microbenchmark, which poses a hard upper bound on how fast \phub can run during training. We also see that, when training VGG with \code{ZeroComputeEngine}, as more workers are added, \phubbox{}'s performance approached the microbenchmarks (97\%), demonstrating \phub{}'s ability to fully utilize system resources. The gap in the plot between \phubbox and the microbenchmark %before they overlap 
is due to the overhead of scheduling operations in \mxnet and straggler effects in workers. \phubbox{} hit the limit at a sustained 80GB/s memory bandwidth.

In real training, however, \phubbox{}'s scalability limit was difficult to reach. Recent work (\cite{keskar2016large, lecun1524efficient}) describes the difficulty of generalization with large batch sizes; it is not advantageous to blindly scale deep learning to a large number of workers without considering statistical efficiency~\cite{youspeeding, koliousiscrossbow}. One example \cite{ImageNetIn1Hour} reports that ResNet 50's statistical efficiency drops with aggregate batch sizes larger than 8192 on a system with 256 GPUs on 32 machines (with a mini-batch size of 32 per GPU). To assess whether \phubbox could reach this scale, we measured the memory bandwidth usage for ResNet 50 with 8 workers using the same batch size. We found that \phubbox required only 6GB/s memory bandwidth and an aggregated 4GB/s network bandwidth. This suggests that our \phubbox prototype could scale to rack-level and support up to 120 worker machines training this network. In other words, our prototype could support sufficient scalability to handle cutting-edge training tasks.

On the other hand, the scalability bottleneck (PCIe controller) in our current prototype is specific to this particular platform, but it can change. For example, recently released AMD Epyc~\cite{AMDEpyc} processors provide nearly triple the Stream Triad performance
(290 GB/s)~\cite{EpycBenchmark} and 40\% more PCIe bandwidth than our
\phubbox machine. We would expect Epyc to support 40\% more
throughput.
%Our test cluster does not have enough machines to saturate either of these, but we can project when scalability will stop based on these limits.


\subsection{Effectiveness of \phubbox as a Rack-Scale Service}
\label{sec:hierarchicalEval}
We now evaluate effectiveness of \phubbox as a rack-scale service with two typical scenarios in a 10 Gbps cloud-like environment: (1) when multiple jobs are training in parallel in a rack, sharing the same \phubbox instance with different key namespaces and (2) when a training job crosses rack boundaries, and \phub performs hierarchical reduction.

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=2 2 2 2,clip]{Figures/MultijobSim.pdf}
	\caption{Overhead of multiple parallel training jobs sharing the same \phubbox instance.}
	\label{fig:multijobs}
\end{figure}

Figure \ref{fig:multijobs} shows the overhead of running multiple independent training jobs when sharing a single \phubbox instance. AlexNet saw a 5\% drop in per-job throughput when running 8 jobs, likely due to frequent invocation of optimizer and less effective caching; ResNet 50 saw a smaller impact as it is compute bound.

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=2 6 2 2,clip]{Figures/HierarchicalSim.pdf}
	\caption{Emulated overhead of hierarchical reduction with \phubbox.}
	\label{fig:hierarchical}
\end{figure}

Figure \ref{fig:hierarchical} emulates the a single cloud-based training job whose VMs span N racks, and each rack contains 8 workers and 1 \phubbox. The \phubbox uses a widely used ring reduction algorithm~\cite{baidures3:online,DBLP:journals/corr/abs-1802-05799} for inter-rack aggregation. 

Since we have only one \phubbox machine, we model this ring reduction by sending and receiving N chunk-size messages sequentially, each performing one additional aggregation, for each of the keys, after local rack has finished aggregation. We assume each rack would finish its local aggregation at roughly the same time, as stragglers can exist regardless of rack assignment. Therefore, this faithfully estimates overhead of \phub{}'s hierarchical reduction.

The lost throughput of AlexNet comes from added latency of multiple rounds of communication, but is compensated by drastically reduced cross-rack communication, and thus we would expect speedup in real deployment. On the other hand, we again observed virtually no loss of throughput in ResNet 50.


==> SOCC 18/HardwarePHUB.tex <==
%\subsection{\phubbox: Balanced Hardware for Efficient Centralized PSs}
%\subsection{\phubbox: A Balanced Hardware Design for Rack-Scale Centralized PSs}
\subsection{A Balanced Hardware Design for Rack-Scale PSs}
%\subsection{\phubbox: Balanced Design for Efficient Centralized PSs}
\label{sec:phub}
Centralized PSs have lower cost than NCS PSs, and half of the bandwidth stress compared to CS PSs on each interface card. Thus it is desirable to have a centralized reduction entity at rack level. However, scaling a centralized PS to rack scale is challenging~\cite{firecaffe}, despite the optimizations in \mysection\ref{sec:commonOptimizations}.
%Because they dedicate their full bandwidth to the PS process, centralized PSs are bandwidth efficient without the extra hardware cost for non-colocated sharded PSs. They are also compute efficient when not overwhelmed~\cite{firecaffe}. However, while optimizations in \mysection\ref{sec:commonOptimizations} benefit sharded servers, they have only limited effect on the throughput of a centralized PS. 
%The root cause is hardware imbalance in resource allocation of the host machine.
The root cause is hardware imbalance in allocation of computation and communication resources in the host machine: centralized PSs usually run on the same hardware configuration as a worker, which have only one or two network interfaces. This implies incast congestion from their high bandwidth usage (Table \ref{table:bwReqDC}) when serving multiple workers, starving the compute units. 

%Hardware imbalances result from vastly different computation and communication resources in a machine, which is in turn related to how centralized PSs are deployed. Centralized PSs usually run on the same hardware as a worker and have only one or two network interfaces. This implies incast congestion from their high bandwidth usage (Table \ref{table:bwReqDC}) when serving multiple workers, starving the compute units. 

%Existing frameworks also cannot efficiently use full hardware, even if multiple interfaces are present (for example, TensorfFlow and \mxnet can only use multiple interfaces by spawning multiple PS processes), let alone understanding the topology of the underlying hardware to balance workload in each interface, processor core and NUMA domain.

One trivial solution would be to simply use interfaces with higher bandwidth. However, even in the best case, a single network interface is not capable of saturating memory or PCIe bandwidth. A single network interface also causes serialization delay and further imbalance across NUMA domains in a typical server. %It is not possible to fully utilize the entire server without balancing these resources.

%The solution may seem trivial: just add more interfaces, or use interfaces with higher capacity. These, however, are not enough. First, most parameter server implementations (TensorFlow, \mxnet and etc) do not allow use of multiple interfaces in a single parameter server process instance. To support that, the software stack must understand the topology of the underlying system and produce a balanced scheme across multiple interfaces with minimum polling overhead; second, existing single interface is unlikely able to match the memory bandwidth nor the PCIe bandwidth, and they can still cause serialization delay, further causing imbalance across NUMA domains on typical server systems.

%Software changes alone is not enough to scale training throughput on a typical centralized parameter server, because the hardware offered is inbalanced itself: the provisioned network bandwidth is vastly smaller than available memory bandwidth.

%Therefore, a hardware design that optimizes balance is needed to fully scale a centralized PS. 
This section describes \phubbox, our \textit{balanced parameter exchange system}. We maintain that a centralized system, when architected properly, can provide high throughput, low latency, sufficient scalability for a rack, and low cost. We prototyped \phubbox using an off-the-shelf server platform that was configured to our requirements. Our goal was to balance IO and memory bandwidth; our prototype system had memory bandwidth of 120 GB/s and theoretical overall bidirectional IO bandwidth of 140 GB/s. To fully utilize resources, \phubbox needed a matching network capability, which we provided by using multiple network interfaces. Figure \ref{fig:phub} shows the resulting \phubbox design. The system includes 10 network interfaces, each of 56 Gbps link speed, connected to a switch. This uses all PCIe bandwidth on our dual socket prototype and provides roughly 136 GB/s bandwidth once IB and PCIe framing overheads are taken into account, balancing IO and memory bandwidth.

\begin{figure}[t!]
	\centering
	\includegraphics[width=.8\linewidth,trim=1 0 1 1,clip]{Figures/PHubOverview.pdf}
	\caption{The \phubbox architecture}
	\label{fig:phub}
\end{figure}

Hardware alone solves only part of the problem. Existing frameworks cannot efficiently use the full hardware capability even if multiple interfaces are present (for example, TensorFlow and \mxnet support multiple interfaces only by spawning multiple PS processes). Thus, software that understands both the hardware topology \textit{and} balance is required to complete the solution. \phub takes full advantage of \phubbox by extending the chunk-to-core mapping scheme (\mysection\ref{sec:chunk2core})%It ensures balance across queue pairs, completion queues, interfaces, cores, and NUMA domains. 
, ensuring balance across interfaces and NUMA domains. \phub further guarantees no inter-processor traffic on \phubbox, and completion queues and queue pairs in an interface card are used by only one core in the same NUMA domain to promote locality and avoid coherence traffic. In essence, \phubbox forms micro-shards inside a box.

%We also tried an alternate chunk-to-core mapping scheme with \phubbox. In this approach, workers, rather than keys, were partitioned across interfaces; each worker sent all its keys through a single \phubbox interface (a ``direct'' connection). While the alternative scheme reduced reception latency, it added synchronization and communication overheads since multiple NUMA nodes participated in aggregating each key. We found this scheme inferior to the original design.


==> SOCC 18/HierarchicalReduction.tex <==
\subsection{Rack Deployment and Topology-Aware Reduction}
\label{sec:hierarchicalReduction}

\begin{figure}[t!]
	\centering
	\includegraphics[width=.7\linewidth,trim=2 1 1 2,clip]{Figures/PBoxDeployment.pdf}
	\caption{\phubbox deployment scheme}
	\label{fig:pBoxDeployment}
\end{figure}

We associate a \phubbox with a ToR during deployment for two reasons. First, full bisection bandwidth is achievable for machines in the same rack, making it ideal for a central reduction entity as \phubbox, while oversubscription occurs between the ToR and the cluster network. Second, as we show in \mysection\ref{sec:scability}, a single \phubbox has enough scalability for a typical rack of worker machines.

When provisioned in each rack (Figure \ref{fig:pBoxDeployment}), \phubbox{}es can form an array of sharded PSs, or run a \textit{hierarchical reduction} algorithm for a training task that spans multiple racks through the coordination of a connection manager. Hierarchical reduction works in three steps: first, each \phubbox centrally aggregates gradient updates from workers in the same rack; then, the \phubbox{} nodes start cross-rack aggregation and compute globally aggregated gradients; finally, each per-rack \phubbox runs an optimizer on this gradient and broadcasts the new weights back to local workers.

Hierarchical reduction trades off more rounds of communication for lower cross-rack traffic ($1/N$ with N-worker racks). \phub determines when hierarchical reduction is potentially beneficial with the simple model below:
%\[	max(\frac{N-1}{B_{bn}}, \frac{1}{B_{Wkr}})  > max(\frac{1}{B_{Wkr}}, \frac{N}{B_{PBox}}) + C\]
\[	max(\frac{N-1}{B_{bn}}, \frac{1}{NB_{Wkr}}) > max(\frac{1}{B_{PBox}}, \frac{N}{B_{Wkr}}) + C\]

where $B_{PBox}, B_{Core}$ and $B_{Wkr}$ are the bandwidths of a \phubbox, the network core, and a worker,  $B_{bn} = min((r-1)B_{PBox}, B_{Core})$, and $r$ is the number of racks. When the condition is true, this means the time to perform cross-rack transfer is larger than the added latency of a two-level reduction, which consists of a per-rack local aggregation that happens in parallel and an inter-rack communication (with cost $C$) done with either sharded PSs ($C=\frac{N-1}{NB_{bn}}$) or a collectives operation (e.g., $C\approx\frac{r-1}{rB_{bn}}$ with racks forming a ring). \mysection\ref{sec:hierarchicalEval} estimates the overhead of $C$, and $B_{Core}$ can be effectively probed by using~\cite{hu2002estimating,hu2003evaluation}.
%>>>>>>> 7a41c5c... rewrote 2.3 and 3.4

%The flexibility of \phub software allows \phubbox to run many forms of hierarchical reduction, cutting cross-rack traffic by N times (where N is the number of workers on each rack) when compared to existing PSs that use a shard or central setup. However, hierarchica reduction trades longer latency for traffic reduction. 


==> SOCC 18/Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
To date, most work in the systems and architecture community has focused on improving the efficiency of evaluating trained models. However, arriving at a trained model frequently requires experimentation, and thus multiple training runs, each of which may take days. Accelerating the training process lets neural network developers iterate faster and design better models.

As DNNs get computationally more expensive to train, timely training requires exploiting parallelism with a distributed system, especially in the cloud~\cite{CloudTPU88:online,MachineL65:online,ApacheMX19:online}. The most common way of exploiting parallelism is called ``data'' parallelism, which consists of a computational-heavy forward and backward phase and a communication-heavy parameter exchange phase.

%DNNs have transformed the field of machine learning, providing state-of-the-art accuracy for a variety of text, speech, image, and audio processing tasks. 
% Fueling the transformation are new techniques, bigger datasets, and greatly increased computational capabilities. These factors are rapidly advancing the field, beating traditional techniques and even humans for some tasks.
%To date, most work in the systems and architecture community has focused on improving the efficiency of evaluating trained models.  %This makes sense given that a model is trained only once but can be used many times for inference. 
%However, arriving at a trained model frequently requires experimentation, and thus multiple training runs, each of which may take days. Accelerating the training process lets neural network developers iterate faster and design better models.

%Traditionally, DNN training has been viewed as a compute-bound problem, best done in a single large compute node with many GPUs. However, as DNNs get computationally more expensive to train, timely training requires exploiting parallelism with a distributed system, especially in the cloud~\cite{CloudTPU88:online,MachineL65:online,ApacheMX19:online}.

%DDNN training has ample parallelism that can be exploited to speed up the training process. %
%Parallelism in the DDNN training process can be decomposed in multiple ways; the most common, known as ``data'' parallelism, gives each worker GPU a complete copy of the model being trained but a different sample of the input data. This lets the forward and backward passes run locally, without communication. Thereafter, gradients are exchanged, the global view of the model is updated in the PS, and the new model parameters are sent back to the workers. Thus, a single iteration of the training process has two main components: a computation-intensive part and a communication-intensive part.

In this paper, we begin by performing a detailed bottleneck analysis of DDNN training and observe that the emergence of speedier accelerators shifts \textit{the performance bottleneck of distributed DNN training from computation to communication}, because of the following factors. 

First, the throughput of GPUs on a recent DNN, ResNet, has increased by 35x since 2012 on modern cloud-based GPUs (Figure~\ref{fig:GPUPower}), effectively demanding a similar increase in network bandwidth, causing bandwidth deficiency.
Upgrading datacenter networks is expensive: compute instance network bandwidth on major cloud providers such as EC2 has improved little across generational upgrades~\cite{ec2BW}, so care must be taken when configuring racks for DDNN training for optimal cost-efficiency.

Second, existing parameter exchange mechanisms such as parameter servers (PS) do not scale up the total throughput on a standard cloud network stack~(Table~\ref{table:frameworkPerf}) due to unoptimized software and hardware configuration, and lack of awareness of the underlying physical network topology. 

The compound effect of these factors dramatically increases communication overhead during distributed DNN training. To illustrate this problem, Figure \ref{fig:IncreasingCommToCompRatio} shows a modest-scale DNN training with 8 machines on EC2 with 10 Gbps links\footnote{%All instances have advertised 10Gbps links, but empirical measurement with iperf shows 7.11Gbps links on GRID 520 instances. %
Batch size per GPU (4, 16, 32, 32, saturating GRID 520) for each network is kept the same across all GPUs for easier comparison.}: modern DNN training frameworks can no longer hide the latency of communication due to faster computation. Spending most of the DDNN training time on model updates limits the benefit of faster GPUs.

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=3 13 3 3,clip]{Figures/GPUPower.pdf}
	%\caption{Single-GPU training throughput for ResNet-269 measured with \mxnet on EC2 g2, p2, g3 and p3 instances, and a local machine (GTX 1080 Ti), while maximizing GPU memory utilization. Per chip GPU throughput on ResNet 269 in the cloud has increased 35x since 2012.}
	\caption{Single-GPU training throughput for ResNet 269 measured with \mxnet on EC2 g2, p2, g3 and p3 instances, and a local GTX 1080 Ti machine, while maximizing GPU memory utilization. Per chip GPU throughput on ResNet 269 in the cloud has increased 35x since 2012.}
	\label{fig:GPUPower}
\end{figure}

\begin{figure}[t!]
	\includegraphics[width=\linewidth,trim=4 13 3 4,clip]{Figures/IncreasingCommToCompRatio.pdf}
	\caption{The overhead of distributed training gets larger as GPUs get faster. The framework can no longer hide communication latency, and faster GPUs no longer improve training throughput. With today's fast GPUs, distributed cloud DNN training time is chiefly spent waiting for parameter exchanges.}
	\label{fig:IncreasingCommToCompRatio}
\end{figure}
 %(even for networks with small models), 
%, most training time is spent waiting for model updates, limiting 
%\footnote{
%One solution is to increase the per-GPU batch size, leading to a large global batch size. Large global batch sizes can reduce statistical efficiency \cite{ImageNetIn1Hour,keskar2016large,lecun1524efficient}; also, GPUs have limited memory.
%Techniques such as \cite{chen2016training} could alleviate that pressure, but with higher
%computational cost.
%}

Scaling cloud-based DDNN training throughput demands both a fast and a cost-effective solution. Our bottleneck findings show that such a solution requires a more optimized software stack, a specialized hardware design, and a more effective cluster configuration.


We therefore propose \phub, a high performance, multi-tenant, rack-scale PS design for cloud-based DDNN training. By co-designing the PS software with the hardware and the datacenter cluster rack configuration, \phub achieves up to 2.7x faster training throughput, with 25\% better throughput per dollar.
Our contributions include:
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
	\item A detailed bottleneck analysis of current state-of-the-art cloud-based DDNN training~(\mysection\ref{sec:background}).
	\item Design and implementation of the \phub PS software, supporting many DNN training frameworks~(\mysection\ref{sec:design}).
	\item A \textit{balanced} central PS hardware architecture, \phubbox(\mysection\ref{sec:phub}), to leverage \phub for rack-level and hierarchical cross-rack gradient reduction.
	\item A comprehensive evaluation of \phub in terms of performance, scalability, and deployment cost~(\mysection\ref{sec:evaluation}).
\end{enumerate}


%In this work, we propose \phub, a holistic parameter server software, hardware and cluster rack configuration co-design (\mysection\ref{sec:design}) that provides high training throughput with low network cost.

%What does this observation mean for operators designing and deploying new training clusters? For dedicated training clusters where minimizing training time is a more important metric than cost, the consequence is clear: operators should deploy the fastest network possible. However, in cloud datacenter environments where the cluster will be rented to customers, cost is a fundamental metric. A practical cluster design must balance performance against cost in order to build a product that is cheap enough for customers to use and flexible enough to support a broad range of workloads.



%To that end,
%To address the growing computation-communication imbalance, we studied the designs of common PSs and characterized DDNN training workloads. 
%We discovered that the main bottlenecks in updating models were insufficient network bandwidth and inefficiencies in the software stack of existing PSs, including large overheads from data copies and suboptimal implementations of aggregation and optimization.
%We observed two key properties. First, from a theoretical perspective, \textit{centralized parameter servers move fewer bytes than sharded parameter servers}, reducing the load on the network and supporting the use of cheaper, low-bandwidth, oversubscribed networks to provide high training throughput. Second, \textit{current cloud server configurations are unbalanced and inefficient for parameter server workloads}: a single server has enough compute capability to scale to very large training jobs, but it does not have enough network bandwidth to keep its CPUs fed.


%\phub consists of three components: an efficient PS software stack with a streamlined gradient processing pipeline; \phubbox,  PS hardware with balanced compute/networking resources; and an API portable to multiple deep learning frameworks that takes advantage of this software/hardware configuration.
%By co-designing the parameter server software with the parameter server hardware and the cluster rack configuration, \phub provides high training throughput with low network cost.


%\phub optimizes the network stack and streamlines the gradient processing pipeline.
%To make full use of \phub's capabilities, we also prototyped \phubbox:


%% Our paper's contributions include:
%% \begin{CompactEnumerate}

%% \item A study of common PS configurations and their tradeoffs, and detailed profiling of cloud-based DDNN training, to identify performance bottlenecks and inefficiencies
%% \item The design and implementation of a new PS architecture, \phub, that delivers up to 3x faster throughput for cloud-based DNN training compared to the state-of-the-art with the same hardware resources, and is compatible with multiple DNN training frameworks
%% \item A new hardware design, \phubbox, that offers further throughput benefits by balancing per-link traffic with computation in the PS
%% %and, \item projections for hardware-based implementations of a Parameter Switch, that does key parts of the computation in a programmable datacenter switch.
%% \end{CompactEnumerate}


% or up to 2.9x when  \TODO{Should we say something about better perf with same compute resources?}

%In the following discussion, \mysection\ref{sec:background} presents background information on DDNN training, surveys popular DDNN training frameworks, and profiles cloud-based DDNN training with \mxnet. We discuss in \mysection\ref{sec:design} \phub{}'s parameter exchange design and the \phubbox hardware. \mysection\ref{sec:evaluation} evaluates our design, and \mysection\ref{sec:discussion} discusses related work. We present concluding remarks in \mysection\ref{sec:conclusion}.



% \TODO{more focus on balance; more references}




==> SOCC 18/Model.tex <==
\subsection{Rack-scale cost model}

Is a cluster built with PHubs and a slow network more cost effective than one with sharded PSs and a fast network? This section explores this question using a simple cost model. We consider the cost of three cluster components: worker nodes, PHub nodes, and network gear. We use advertised prices from the Internet; while a datacenter operator might pay less, the ratios between component prices should still be similar. The baseline is a cluster running MXNet IB with colocated sharded PSs; we compare this to a PHub deployment in terms of throughput per dollar.

The model works by computing the cost of a worker node, and adding to it the amortized cost of its network usage; for the PHub deployment, it also includes the amortized cost of the worker's PHub usage. This allows us to compare the cost of worker nodes in deployments with different numbers of workers per rack, switch, or PHub. We capture only the most significant cost, and include only capital cost, since operational costs are dominated by GPU power usage and thus differences would be small.

We model a standard three-layer datacenter network with some simplifying assumptions: racks hold as many machines as may be connected to a single switch, all switches and cables are identical, and oversubscription happens only at ToR switches. We model network costs by charging each worker the NIC per-port cost $N$, the amortized cost of one ToR switch port $S$ and cable $C$, and fractional costs of ToR/aggregation/core switch ports and cables depending on the oversubscription factor $F$. Thus, the amortized cost of the network per machine is $A=(N+S+C)+F(4S+2C)$. 

Since our goal is to model costs for future deployments, we make two changes from our experimental setup. Instead of 10Gb IB, we use 25 Gb Ethernet. Instead of NVIDIA 1080 Ti's, we assume a future, faster GPU with similar cost $G$, but performance like today's V100. Based on the data in Figure~\ref{fig:gpuPower}, this keeps the compute/communication ratio similar to that of our experiments. We use ResNet-50 for comparison; we use our 10Gb IB results for the PHub setting and downclocked 40Gb IB for the MXNet IB baseline. We include 2\% overhead in the PHub numbers to account for aggregation between racks.

%We use similar worker and PHub nodes as in our experiments. The cost $W$ is 

%% For the baseline, we use the same SuperMicro 1028GQ-TR worker nodes as in our evaluation, but with 4 GPUs. The advertised cost $W$ is \$4117~\cite{worker-price} without GPUs; we use the price of the NVIDIA GeForce 1080 Ti (\$699~\cite{nvidia-1080ti}) for the GPU price $G$. We use the Mellanox ConnectX-4 EN for 100Gb Ethernet (\$795~\cite{mellanox-eth}); the cost of a 2 meter cable is \$94~\cite{mellanox-cable}. The PHub worker nodes have the same configuration but with Mellanox ConnectX-4 Lx EN cards for 25Gb Ethernet (\$260~\cite{mellanox-eth}); the cable cost is \$31.25 using 4-to-1 breakout cables~\cite{mellanox-cable}. The PHub node is the same SuperMicro 6038R-TXR as in the evaluation; its cost $H$ is \$8407~\cite{phub-price}, and it uses 10 dual-port 25Gb Mellanox ConnectX-4 Lx EN cards (\$325~\cite{mellanox-eth}, or \$162.5 per port). We use the Arista 7060CX-32S 32-port 100Gb Ethernet switch (\$21077~\cite{}) in both configurations, with breakout cables to connect the 25Gb hosts. This means that with no oversubscription, a single switch can support 16 100Gb baseline workers, or a PHub and 44 25Gb workers. We assume 1 PHub per switch to allow for oversubscription; with 2:1 oversubscription each switch could support 65 25Gb workers; with 3:1 oversubscription, 76. The cost of each baseline worker is $W+N+4G+A$, and the cost of a PHub worker is $W+N+4G+A+KP$, where $KP$ is the amortized cost of the PHub ($P=W+20N$ and $K$ is the worker-to-phub ratio).

Workers are the same as in our evaluation, but with 4 GPUs. The cost $W$ is \$4117~\cite{worker-price} without GPUs; the GPU price $G$ is (\$699~\cite{nvidia-1080ti}). The 100Gb baseline uses Mellanox ConnectX-4 EN cards (\$795~\cite{mellanox-eth}) and 2m cables (\$94~\cite{mellanox-cable}). The 25Gb PHub workers use Mellanox ConnectX-4 Lx EN cards (\$260~\cite{mellanox-eth}) and 4-to-1 breakout cables (\$31.25 per port~\cite{mellanox-cable}).
The PHub node (also same as evaluation) cost $H$ is \$8407~\cite{phub-price}, plus 10 dual-port 25Gb Mellanox ConnectX-4 Lx EN cards (\$162.5 per port~\cite{mellanox-eth}). The cost of each baseline worker is $W+N+4G+A$, and the cost of a PHub worker is $W+N+4G+A+KP$, where $KP$ is the amortized PHub cost ($P=W+20N+20A$; $K$ is the worker to \phub ratio).

We use the Arista 7060CX-32S 32-port 100Gb Ethernet switch (\$21077~\cite{arista-price}) in both configurations, with breakout cables to connect 25Gb hosts.
With no oversubscription, each switch supports 16 100Gb baseline workers, or a PHub and 44 25Gb workers. With 2:1 oversubscription each switch could support a \phub and 65 25Gb workers; with 3:1, 76. 




%% \begin{table}[tb!]
%%   \centering
%%   \small
%%   \begin{tabular}{|r|c|c|c|}
%%     \hline
%%                   & Baseline         & PHub worker                & PHub \\
%%     \hline
%%     $W$ & \$4117~\cite{worker-price} & \$4117~\cite{worker-price} & \$8407~\cite{phub-price} \\
%%     $G$ & \$699~\cite{nvidia-1080ti} & \$699                      & \\
%%     $N$ & \$795~\cite{mellanox-eth}  & \$260                      & \$162.5/port \\
%%     $S$ & \$795~\cite{mellanox-eth}  & \$260                      & \$162.5/port \\
%%     \hline
%%   \end{tabular}
%%   \caption{Cost model parameters}
%%   \label{table:costModelParam}
%% \end{table}

\begin{table}[tb!]
  \centering
  \footnotesize
  \begin{tabular}{|r|c|c|c|}
    \hline
    & \multicolumn{3}{c|}{Throughput/\$1000} \\
                                 & Future GPUs & Spendy & Cheap \\
    \hline
    100Gb Sharded 1:1 &             46.11 &          14.57 &      60.41\\
    \hline 
    25Gb PHub     1:1 &             55.19 &          15.30 &      77.21\\
    \hline 
    25Gb PHub     2:1 &             57.71 &          15.49 &      82.24\\
    \hline 
    25Gb PHub     3:1 &             59.03 &          15.58 &      84.95\\
    \hline
  \end{tabular}
  \caption{Datacenter cost model comparing 25GbE PHub deployments with 100GbE MXNet IB on ResNet-50. Higher is better. The Future GPU PHub deployment with 2:1 oversubscription provides 25\% better throughput per dollar.}
  \label{table:costModel}
\end{table}

%% Table~\ref{table:costModel} compares a full-bisection-bandwidth 100GbE sharded MXNet IB deployment with 25GbE PHub deployments with varying oversubscription. With 2:1 oversubscription, the PHub deployment provides 26\% better throughput per dollar. We consider two other configurations. First, one using today's expensive V100s, where the 2:1 PHub deployment provides only 6\% better throughput per dollar: future GPUs this expensive are likely to be faster than this, so this configuration essentially provides a lower bound to improvement. Second, one using cheap (E5-2603 v4) in workers, providing 38\% better throughput per dollar: since the majority of training is done on the GPUs, CPU performance may not be important.

Table~\ref{table:costModel} compares a full-bisection-bandwidth 100GbE sharded MXNet IB deployment with 25GbE PHub deployments with varying oversubscription. With 2:1 oversubscription, the PHub deployment provides 26\% better throughput per dollar. We consider two other configurations: first, a ``lower bound'' using today's expensive V100's, where the 2:1 PHub deployment provides only 6\% improvement; and a ``GPU-focused'' one using cheap CPUs (E5-2603 v4) in workers, providing 36\% improvement.







==> SOCC 18/packages.tex <==
\usepackage{amsmath}
%\usepackage[hyphens]{url}
\usepackage{url}
\usepackage{graphicx}
\usepackage{color}
\usepackage{booktabs}
\usepackage[normalem]{ulem}
\usepackage{wasysym}
\usepackage{microtype}
\usepackage{wasysym}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{authblk}
\usepackage{enumitem}
\usepackage{verbatim}
\usepackage{tabularx}
%\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
\usepackage{amsmath}

